The Deep and Transient Universe in the SVOM Era: New Challenges and Opportunities - Scientific prospects of the SVOM mission

To take advantage of the astrophysical potential of Gamma-Ray Bursts (GRBs), Chinese and French astrophysicists have engaged the SVOM mission (Space-based multi-band astronomical Variable Objects Monitor). Major advances in GRB studies resulting from the synergy between space and ground observations, the SVOM mission implements space and ground instrumentation. The scientific objectives of the mission put a special emphasis on two categories of GRBs: very distant GRBs at z$>$5 which constitute exceptional cosmological probes, and faint/soft nearby GRBs which allow probing the nature of the progenitors and the physics at work in the explosion. These goals have a major impact on the design of the mission: the on-board hard X-ray imager is sensitive down to 4 keV and computes on line image and rate triggers, and the follow-up telescopes on the ground are sensitive in the NIR. At the beginning of the next decade, SVOM will be the main provider of GRB positions and spectral parameters on very short time scale. The SVOM instruments will operate simultaneously with a wide range of powerful astronomical devices. This rare instrumental conjunction, combined with the relevance of the scientific topics connected with GRB studies, warrants a remarkable scientific return for SVOM. In addition, the SVOM instrumentation, primarily designed for GRB studies, composes a unique multi-wavelength observatory with rapid slew capability that will find multiple applications for the whole astronomy community beyond the specific objectives linked to GRBs. This report lists the scientific themes that will benefit from observations made with SVOM, whether they are specific GRB topics, or more generally all the issues that can take advantage of the multi-wavelength capabilities of SVOM.

==> whitepaper_v20_bbl.tex <==
%\begin{thebibliography}{}
%\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi

\bibitem[{Aab {et~al.}(2015)}]{Auger2015}
Aab, A., {et~al.} 2015, Phys. Rev., D91, 092008

\bibitem[{{Aartsen} {et~al.}(2014{\natexlab{a}}){Aartsen}, {Ackermann},
  {Adams}, {Aguilar}, {Ahlers}, {Ahrens}, {Altmann}, {Anderson}, {Arguelles},
  {Arlen}, \& et~al.}]{Aartsen2014}
{Aartsen}, M.~G., {Ackermann}, M., {Adams}, J., {et~al.} 2014{\natexlab{a}},
  Physical Review Letters, 113, 101101

\bibitem[{{Aartsen} {et~al.}(2014{\natexlab{b}}){Aartsen}, {Ackermann},
  {Adams}, {Aguilar}, {Ahlers}, {Ahrens}, {Altmann}, {Anderson}, {Arguelles},
  {Arlen}, \& et~al.}]{IceCube2014}
---. 2014{\natexlab{b}}, Physical Review Letters, 113, 101101

\bibitem[{{Aartsen} {et~al.}(2015{\natexlab{a}}){Aartsen}, {Abraham},
  {Ackermann}, {Adams}, {Aguilar}, {Ahlers}, {Ahrens}, {Altmann}, {Anderson},
  {Archinger}, \& et~al.}]{aartsen2015bis}
{Aartsen}, M.~G., {Abraham}, K., {Ackermann}, M., {et~al.} 2015{\natexlab{a}},
  Physical Review Letters, 115, 081102

\bibitem[{{Aartsen} {et~al.}(2015{\natexlab{b}}){Aartsen}, {Abraham},
  {Ackermann}, {Adams}, {Aguilar}, {Ahlers}, {Ahrens}, {Altmann}, {Anderson},
  {Archinger}, \& et~al.}]{IceCube2015}
---. 2015{\natexlab{b}}, \apj, 811, 52

\bibitem[{Aasi {et~al.}(2013)}]{Aasi:2013wya}
Aasi, J., {et~al.} 2013, arXiv:1304.0670, [Living Rev. Rel.19,1(2016)]

\bibitem[{{Abbasi} {et~al.}(2010){Abbasi}, {Abdou}, {Abu-Zayyad}, {Adams},
  {Aguilar}, {Ahlers}, {Andeen}, {Auffenberg}, {Bai}, {Baker}, \&
  et~al.}]{Abbasi2010}
{Abbasi}, R., {Abdou}, Y., {Abu-Zayyad}, T., {et~al.} 2010, \apj, 710, 346

\bibitem[{{Abbott} {et~al.}(2016{\natexlab{a}}){Abbott}, {Abbott}, {Abbott},
  {Abernathy}, {Acernese}, {Ackley}, {Adams}, {Adams}, {Addesso}, {Adhikari},
  \& et~al.}]{abbott:2016a}
{Abbott}, B.~P., {Abbott}, R., {Abbott}, T.~D., {et~al.} 2016{\natexlab{a}},
  Physical Review Letters, 116, 131102

\bibitem[{{Abbott} {et~al.}(2016{\natexlab{b}}){Abbott}, {Abbott}, {Abbott},
  {Abernathy}, {Acernese}, {Ackley}, {Adams}, {Adams}, {Addesso}, {Adhikari},
  \& et~al.}]{Abbott:2016}
---. 2016{\natexlab{b}}, Physical Review Letters, 116, 061102

\bibitem[{{Abbott} {et~al.}(2016{\natexlab{c}}){Abbott}, {Abbott}, {Abbott},
  {Abernathy}, {Acernese}, {Ackley}, {Adams}, {Adams}, {Addesso}, {Adhikari},
  \& et~al.}]{2016PhRvL.116f1102A}
---. 2016{\natexlab{c}}, Physical Review Letters, 116, 061102

\bibitem[{{Abbott} {et~al.}(2016{\natexlab{d}}){Abbott}, {Abbott}, {Abbott},
  {Abernathy}, {Acernese}, {Ackley}, {Adams}, {Adams}, {Addesso}, {Adhikari},
  \& et~al.}]{abbott:2016b}
---. 2016{\natexlab{d}}, Living Reviews in Relativity, 19, arXiv:1304.0670

\bibitem[{{Abdo} {et~al.}(2009){Abdo}, {Ackermann}, {Ajello}, {Asano},
  {Atwood}, {Axelsson}, {Baldini}, {Ballet}, {Barbiellini}, {Baring},
  {Bastieri}, {Bechtol}, {Bellazzini}, {Berenji}, {Bhat}, {Bissaldi},
  {Blandford}, {Bloom}, {Bonamente}, {Borgland}, {Bouvier}, {Bregeon}, {Brez},
  {Briggs}, {Brigida}, {Bruel}, {Burgess}, {Burrows}, {Buson}, {Caliandro},
  {Cameron}, {Caraveo}, {Casandjian}, {Cecchi}, {{\c C}elik}, {Chekhtman},
  {Cheung}, {Chiang}, {Ciprini}, {Claus}, {Cohen-Tanugi}, {Cominsky},
  {Connaughton}, {Conrad}, {Cutini}, {d'Elia}, {Dermer}, {de Angelis}, {de
  Palma}, {Digel}, {Dingus}, {Silva}, {Drell}, {Dubois}, {Dumora}, {Farnier},
  {Favuzzi}, {Fegan}, {Finke}, {Fishman}, {Focke}, {Fortin}, {Frailis},
  {Fukazawa}, {Funk}, {Fusco}, {Gargano}, {Gehrels}, {Germani}, {Giavitto},
  {Giebels}, {Giglietto}, {Giordano}, {Glanzman}, {Godfrey}, {Goldstein},
  {Granot}, {Greiner}, {Grenier}, {Grove}, {Guillemot}, {Guiriec}, {Hanabata},
  {Harding}, {Hayashida}, {Hays}, {Horan}, {Hughes}, {Jackson},
  {J{\'o}hannesson}, {Johnson}, {Johnson}, {Johnson}, {Kamae}, {Katagiri},
  {Kataoka}, {Kawai}, {Kerr}, {Kippen}, {Kn{\"o}dlseder}, {Kocevski}, {Komin},
  {Kouveliotou}, {Kuss}, {Lande}, {Latronico}, {Lemoine-Goumard}, {Longo},
  {Loparco}, {Lott}, {Lovellette}, {Lubrano}, {Madejski}, {Makeev},
  {Mazziotta}, {McBreen}, {McEnery}, {McGlynn}, {Meegan}, {M{\'e}sz{\'a}ros},
  {Meurer}, {Michelson}, {Mitthumsiri}, {Mizuno}, {Moiseev}, {Monte},
  {Monzani}, {Moretti}, {Morselli}, {Moskalenko}, {Murgia}, {Nakamori},
  {Nolan}, {Norris}, {Nuss}, {Ohno}, {Ohsugi}, {Omodei}, {Orlando}, {Ormes},
  {Paciesas}, {Paneque}, {Panetta}, {Pelassa}, {Pepe}, {Pesce-Rollins},
  {Petrosian}, {Piron}, {Porter}, {Preece}, {Rain{\`o}}, {Rando}, {Rau},
  {Razzano}, {Razzaque}, {Reimer}, {Reimer}, {Reposeur}, {Ritz}, {Rochester},
  {Rodriguez}, {Roming}, {Roth}, {Ryde}, {Sadrozinski}, {Sanchez}, {Sander},
  {Saz Parkinson}, {Scargle}, {Schalk}, {Sgr{\`o}}, {Siskind}, {Smith},
  {Spinelli}, {Stamatikos}, {Stecker}, {Stratta}, {Strickman}, {Suson},
  {Swenson}, {Tajima}, {Takahashi}, {Tanaka}, {Thayer}, {Thayer}, {Thompson},
  {Tibaldo}, {Torres}, {Tosti}, {Tramacere}, {Uchiyama}, {Uehara}, {Usher},
  {van der Horst}, {Vasileiou}, {Vilchez}, {Vitale}, {von Kienlin}, {Waite},
  {Wang}, {Wilson-Hodge}, {Winer}, {Wood}, {Yamazaki}, {Ylinen}, \&
  {Ziegler}}]{2009ApJ...706L.138A}
{Abdo}, A.~A., {Ackermann}, M., {Ajello}, M., {et~al.} 2009, \apjl, 706, L138

\bibitem[{{Abeysekara} {et~al.}(2012){Abeysekara}, {Aguilar}, {Aguilar},
  {Alfaro}, {Almaraz}, {{\'A}lvarez}, {{\'A}lvarez-Romero}, {{\'A}lvarez},
  {Arceo}, {Arteaga-Vel{\'a}zquez}, {Badillo}, {Barber}, {Baughman},
  {Bautista-Elivar}, {Belmont}, {Ben{\'{\i}}tez}, {BenZvi}, {Berley}, {Bernal},
  {Bonamente}, {Braun}, {Caballero-Lopez}, {Cabrera}, {Carrami{\~n}ana},
  {Carrasco}, {Castillo}, {Chambers}, {Conde}, {Condreay}, {Cotti}, {Cotzomi},
  {D'Olivo}, {de la Fuente}, {De Le{\'o}n}, {Delay}, {Delepine}, {DeYoung},
  {Diaz}, {Diaz-Cruz}, {Dingus}, {Duvernois}, {Edmunds}, {Ellsworth}, {Fick},
  {Fiorino}, {Flandes}, {Fraija}, {Galindo}, {Garc{\'{\i}}a-Luna},
  {Garc{\'{\i}}a-Torales}, {Garfias}, {Gonz{\'a}lez}, {Gonz{\'a}lez},
  {Goodman}, {Grabski}, {Gussert}, {Guzm{\'a}n-Ceron}, {Hampel-Arias},
  {Harris}, {Hays}, {Hernandez-Cervantes}, {H{\"u}ntemeyer}, {Imran},
  {Iriarte}, {Jimenez}, {Karn}, {Kelley-Hoskins}, {Kieda}, {Langarica}, {Lara},
  {Lauer}, {Lee}, {Linares}, {Linnemann}, {Longo}, {Luna-Garc{\'{\i}}a},
  {Mart{\'{\i}}nez}, {Mart{\'{\i}}nez}, {Mart{\'{\i}}nez}, {Mart{\'{\i}}nez},
  {Mart{\'{\i}}nez-Castro}, {Martos}, {Matthews}, {McEnery}, {Medina-Tanco},
  {Mendoza-Torres}, {Miranda-Romagnoli}, {Montaruli}, {Moreno}, {Mostafa},
  {Napsuciale}, {Nava}, {Nellen}, {Newbold}, {Noriega-Papaqui},
  {Oceguera-Becerra}, {Olmos Tapia}, {Orozco}, {P{\'e}rez},
  {P{\'e}rez-P{\'e}rez}, {Perkins}, {Pretz}, {Ramirez}, {Ram{\'{\i}}rez},
  {Rebello}, {Renter{\'{\i}}a}, {Reyes}, {Rosa-Gonz{\'a}lez}, {Rosado}, {Ryan},
  {Sacahui}, {Salazar}, {Salesa}, {Sandoval}, {Santos}, {Schneider}, {Shoup},
  {Silich}, {Sinnis}, {Smith}, {Sparks}, {Springer}, {Su{\'a}rez}, {Suarez},
  {Taboada}, {Tellez}, {Tenorio-Tagle}, {Tepe}, {Toale}, {Tollefson}, {Torres},
  {Ukwatta}, {Valdes-Galicia}, {Vanegas}, {Vasileiou}, {V{\'a}zquez},
  {V{\'a}zquez}, {Villase{\~n}or}, {Wall}, {Walters}, {Warner}, {Westerhoff},
  {Wisher}, {Wood}, {Yodh}, {Zaborov}, \& {Zepeda}}]{Abeysekara2012}
{Abeysekara}, A.~U., {Aguilar}, J.~A., {Aguilar}, S., {et~al.} 2012,
  Astroparticle Physics, 35, 641

\bibitem[{{Ackermann} {et~al.}(2010){Ackermann}, {Asano}, {Atwood}, {Axelsson},
  {Baldini}, {Ballet}, {Barbiellini}, {Baring}, {Bastieri}, {Bechtol},
  {Bellazzini}, {Berenji}, {Bhat}, {Bissaldi}, {Blandford}, {Bloom},
  {Bonamente}, {Borgland}, {Bouvier}, {Bregeon}, {Brez}, {Briggs}, {Brigida},
  {Bruel}, {Buson}, {Caliandro}, {Cameron}, {Caraveo}, {Carrigan},
  {Casandjian}, {Cecchi}, {{\c C}elik}, {Charles}, {Chiang}, {Ciprini},
  {Claus}, {Cohen-Tanugi}, {Connaughton}, {Conrad}, {Dermer}, {de Palma},
  {Dingus}, {Silva}, {Drell}, {Dubois}, {Dumora}, {Farnier}, {Favuzzi},
  {Fegan}, {Finke}, {Focke}, {Frailis}, {Fukazawa}, {Fusco}, {Gargano},
  {Gasparrini}, {Gehrels}, {Germani}, {Giglietto}, {Giordano}, {Glanzman},
  {Godfrey}, {Granot}, {Grenier}, {Grondin}, {Grove}, {Guiriec}, {Hadasch},
  {Harding}, {Hays}, {Horan}, {Hughes}, {J{\'o}hannesson}, {Johnson}, {Kamae},
  {Katagiri}, {Kataoka}, {Kawai}, {Kippen}, {Kn{\"o}dlseder}, {Kocevski},
  {Kouveliotou}, {Kuss}, {Lande}, {Latronico}, {Lemoine-Goumard}, {Llena
  Garde}, {Longo}, {Loparco}, {Lott}, {Lovellette}, {Lubrano}, {Makeev},
  {Mazziotta}, {McEnery}, {McGlynn}, {Meegan}, {M{\'e}sz{\'a}ros}, {Michelson},
  {Mitthumsiri}, {Mizuno}, {Moiseev}, {Monte}, {Monzani}, {Moretti},
  {Morselli}, {Moskalenko}, {Murgia}, {Nakajima}, {Nakamori}, {Nolan},
  {Norris}, {Nuss}, {Ohno}, {Ohsugi}, {Omodei}, {Orlando}, {Ormes}, {Ozaki},
  {Paciesas}, {Paneque}, {Panetta}, {Parent}, {Pelassa}, {Pepe},
  {Pesce-Rollins}, {Piron}, {Preece}, {Rain{\`o}}, {Rando}, {Razzano},
  {Razzaque}, {Reimer}, {Ritz}, {Rodriguez}, {Roth}, {Ryde}, {Sadrozinski},
  {Sander}, {Scargle}, {Schalk}, {Sgr{\`o}}, {Siskind}, {Smith}, {Spandre},
  {Spinelli}, {Stamatikos}, {Stecker}, {Strickman}, {Suson}, {Tajima},
  {Takahashi}, {Takahashi}, {Tanaka}, {Thayer}, {Thayer}, {Thompson},
  {Tibaldo}, {Toma}, {Torres}, {Tosti}, {Tramacere}, {Uchiyama}, {Uehara},
  {Usher}, {van der Horst}, {Vasileiou}, {Vilchez}, {Vitale}, {von Kienlin},
  {Waite}, {Wang}, {Wilson-Hodge}, {Winer}, {Wu}, {Yamazaki}, {Yang}, {Ylinen},
  \& {Ziegler}}]{2010ApJ...716.1178A}
{Ackermann}, M., {Asano}, K., {Atwood}, W.~B., {et~al.} 2010, \apj, 716, 1178

\bibitem[{{Ackermann} {et~al.}(2013{\natexlab{a}}){Ackermann}, {Ajello},
  {Allafort}, {Atwood}, {Baldini}, {Ballet}, {Barbiellini}, {Bastieri},
  {Bechtol}, {Belfiore}, {Bellazzini}, {Bernieri}, {Bissaldi}, {Bloom},
  {Bonamente}, {Brandt}, {Bregeon}, {Brigida}, {Bruel}, {Buehler}, {Burnett},
  {Buson}, {Caliandro}, {Cameron}, {Campana}, {Caraveo}, {Casandjian},
  {Cavazzuti}, {Cecchi}, {Charles}, {Chaves}, {Chekhtman}, {Cheung}, {Chiang},
  {Chiaro}, {Ciprini}, {Claus}, {Cohen-Tanugi}, {Cominsky}, {Conrad}, {Cutini},
  {D'Ammando}, {de Angelis}, {de Palma}, {Dermer}, {Desiante}, {Digel}, {Di
  Venere}, {Drell}, {Drlica-Wagner}, {Favuzzi}, {Fegan}, {Ferrara}, {Focke},
  {Fortin}, {Franckowiak}, {Funk}, {Fusco}, {Gargano}, {Gasparrini}, {Gehrels},
  {Germani}, {Giglietto}, {Giommi}, {Giordano}, {Giroletti}, {Godfrey},
  {Gomez-Vargas}, {Grenier}, {Guiriec}, {Hadasch}, {Hanabata}, {Harding},
  {Hayashida}, {Hays}, {Hewitt}, {Hill}, {Horan}, {Hughes}, {Jogler},
  {J{\'o}hannesson}, {Johnson}, {Johnson}, {Johnson}, {Kamae}, {Kataoka},
  {Kawano}, {Kn{\"o}dlseder}, {Kuss}, {Lande}, {Larsson}, {Latronico},
  {Lemoine-Goumard}, {Longo}, {Loparco}, {Lott}, {Lovellette}, {Lubrano},
  {Massaro}, {Mayer}, {Mazziotta}, {McEnery}, {Mehault}, {Michelson}, {Mizuno},
  {Moiseev}, {Monzani}, {Morselli}, {Moskalenko}, {Murgia}, {Nemmen}, {Nuss},
  {Ohsugi}, {Okumura}, {Orienti}, {Ormes}, {Paneque}, {Perkins},
  {Pesce-Rollins}, {Piron}, {Pivato}, {Porter}, {Rain{\`o}}, {Razzano},
  {Reimer}, {Reimer}, {Reposeur}, {Ritz}, {Romani}, {Roth}, {Saz Parkinson},
  {Schulz}, {Sgr{\`o}}, {Siskind}, {Smith}, {Spandre}, {Spinelli}, {Stawarz},
  {Strong}, {Suson}, {Takahashi}, {Thayer}, {Thayer}, {Thompson}, {Tibaldo},
  {Tinivella}, {Torres}, {Tosti}, {Troja}, {Uchiyama}, {Usher},
  {Vandenbroucke}, {Vasileiou}, {Vianello}, {Vitale}, {Werner}, {Winer},
  {Wood}, \& {Wood}}]{2013ApJS..209...34A}
{Ackermann}, M., {Ajello}, M., {Allafort}, A., {et~al.} 2013{\natexlab{a}},
  \apjs, 209, 34

\bibitem[{{Ackermann} {et~al.}(2013{\natexlab{b}}){Ackermann}, {Ajello},
  {Asano}, {Axelsson}, {Baldini}, {Ballet}, {Barbiellini}, {Bastieri},
  {Bechtol}, {Bellazzini}, {Bhat}, {Bissaldi}, {Bloom}, {Bonamente}, {Bonnell},
  {Bouvier}, {Brandt}, {Bregeon}, {Brigida}, {Bruel}, {Buehler}, {Burgess},
  {Buson}, {Byrne}, {Caliandro}, {Cameron}, {Caraveo}, {Cecchi}, {Charles},
  {Chaves}, {Chekhtman}, {Chiang}, {Chiaro}, {Ciprini}, {Claus},
  {Cohen-Tanugi}, {Connaughton}, {Conrad}, {Cutini}, {D'Ammando}, {de Angelis},
  {de Palma}, {Dermer}, {Desiante}, {Digel}, {Dingus}, {Di Venere}, {Drell},
  {Drlica-Wagner}, {Dubois}, {Favuzzi}, {Ferrara}, {Fitzpatrick}, {Foley},
  {Franckowiak}, {Fukazawa}, {Fusco}, {Gargano}, {Gasparrini}, {Gehrels},
  {Germani}, {Giglietto}, {Giommi}, {Giordano}, {Giroletti}, {Glanzman},
  {Godfrey}, {Goldstein}, {Granot}, {Grenier}, {Grove}, {Gruber}, {Guiriec},
  {Hadasch}, {Hanabata}, {Hayashida}, {Horan}, {Hou}, {Hughes}, {Inoue},
  {Jackson}, {Jogler}, {J{\'o}hannesson}, {Johnson}, {Johnson}, {Kamae},
  {Kataoka}, {Kawano}, {Kippen}, {Kn{\"o}dlseder}, {Kocevski}, {Kouveliotou},
  {Kuss}, {Lande}, {Larsson}, {Latronico}, {Lee}, {Longo}, {Loparco},
  {Lovellette}, {Lubrano}, {Massaro}, {Mayer}, {Mazziotta}, {McBreen},
  {McEnery}, {McGlynn}, {Michelson}, {Mizuno}, {Moiseev}, {Monte}, {Monzani},
  {Moretti}, {Morselli}, {Murgia}, {Nemmen}, {Nuss}, {Nymark}, {Ohno},
  {Ohsugi}, {Omodei}, {Orienti}, {Orlando}, {Paciesas}, {Paneque}, {Panetta},
  {Pelassa}, {Perkins}, {Pesce-Rollins}, {Piron}, {Pivato}, {Porter}, {Preece},
  {Racusin}, {Rain{\`o}}, {Rando}, {Rau}, {Razzano}, {Razzaque}, {Reimer},
  {Reimer}, {Reposeur}, {Ritz}, {Romoli}, {Roth}, {Ryde}, {Saz Parkinson},
  {Schalk}, {Sgr{\`o}}, {Siskind}, {Sonbas}, {Spandre}, {Spinelli}, {Suson},
  {Tajima}, {Takahashi}, {Takeuchi}, {Tanaka}, {Thayer}, {Thayer}, {Thompson},
  {Tibaldo}, {Tierney}, {Tinivella}, {Torres}, {Tosti}, {Troja}, {Tronconi},
  {Usher}, {Vandenbroucke}, {van der Horst}, {Vasileiou}, {Vianello}, {Vitale},
  {von Kienlin}, {Winer}, {Wood}, {Wood}, {Xiong}, \& {Yang}}]{Ackermann2013}
{Ackermann}, M., {Ajello}, M., {Asano}, K., {et~al.} 2013{\natexlab{b}}, \apjs,
  209, 11

\bibitem[{{Adri{\'a}n-Mart{\'{\i}}nez}
  {et~al.}(2013){Adri{\'a}n-Mart{\'{\i}}nez}, {Albert}, {Samarai}, {Andr{\'e}},
  {Anghinolfi}, {Anton}, {Anvar}, {Ardid}, {Astraatmadja}, {Aubert}, {Baret},
  {Barrios-Marti}, {Basa}, {Bertin}, {Biagi}, {Bigongiari}, {Bogazzi},
  {Bouhou}, {Bouwhuis}, {Brunner}, {Busto}, {Capone}, {Caramete},
  {C{\^a}rloganu}, {Carr}, {Cecchini}, {Charif}, {Charvis}, {Chiarusi},
  {Circella}, {Classen}, {Coniglione}, {Core}, {Costantini}, {Coyle},
  {Creusot}, {Curtil}, {De Bonis}, {Dekeyser}, {Deschamps}, {Distefano},
  {Donzaud}, {Dornic}, {Dorosti}, {Drouhin}, {Dumas}, {Eberl}, {Emanuele},
  {Enzenh{\"o}fer}, {Ernenwein}, {Escoffier}, {Fehn}, {Fermani}, {Flaminio},
  {Folger}, {Fritsch}, {Fusco}, {Galat{\`a}}, {Gay}, {Gei{\ss}els{\"o}der},
  {Geyer}, {Giacomelli}, {Giordano}, {Gleixner}, {G{\'o}mez-Gonz{\'a}lez},
  {Graf}, {Guillard}, {van Haren}, {Heijboer}, {Hello}, {Hern{\'a}ndez-Rey},
  {Herold}, {H{\"o}{\ss}l}, {James}, {de Jong}, {Kadler}, {Kalekin}, {Kappes},
  {Katz}, {Kooijman}, {Kouchner}, {Kreykenbohm}, {Kulikovskiy}, {Lahmann},
  {Lambard}, {Lambard}, {Larosa}, {Lef{\`e}vre}, {Leonora}, {Lo Presti},
  {Loehner}, {Loucatos}, {Louis}, {Mangano}, {Marcelin}, {Margiotta},
  {Mart{\'{\i}}nez-Mora}, {Martini}, {Michael}, {Montaruli}, {Morganti},
  {M{\"u}ller}, {Neff}, {Nezri}, {Palioselitis}, {P{\u a}v{\u a}la{\c s}},
  {Perrina}, {Piattelli}, {Popa}, {Pradier}, {Racca}, {Riccobene}, {Richter},
  {Rivi{\`e}re}, {Robert}, {Roensch}, {Rostovtsev}, {Samtleben}, {Sanguineti},
  {Schmid}, {Schnabel}, {Schulte}, {Sch{\"u}ssler}, {Seitz}, {Shanidze},
  {Sieger}, {Simeone}, {Spies}, {Spurio}, {Steijger}, {Stolarczyk},
  {S{\'a}nchez-Losa}, {Taiuti}, {Tamburini}, {Tayalati}, {Trovato}, {Vallage},
  {Vall{\'e}e}, {Van Elewyck}, {Vernin}, {Visser}, {Wagner}, {Wilms}, {de
  Wolf}, {Yatkin}, {Yepes}, {Zornoza}, {Z{\'u}{\~n}iga}, \&
  {Baerwald}}]{Antares2013}
{Adri{\'a}n-Mart{\'{\i}}nez}, S., {Albert}, A., {Samarai}, I.~A., {et~al.}
  2013, \aap, 559, A9

\bibitem[{{Adri{\'a}n-Mart{\'{\i}}nez}
  {et~al.}(2016{\natexlab{a}}){Adri{\'a}n-Mart{\'{\i}}nez}, {Ageron},
  {Aharonian}, {Aiello}, {Albert}, {Ameli}, {Anassontzis}, {Andre},
  {Androulakis}, {Anghinolfi}, \& et~al.}]{Km3net2016}
{Adri{\'a}n-Mart{\'{\i}}nez}, S., {Ageron}, M., {Aharonian}, F., {et~al.}
  2016{\natexlab{a}}, ArXiv e-prints, arXiv:1601.07459

\bibitem[{{Adri{\'a}n-Mart{\'{\i}}nez}
  {et~al.}(2016{\natexlab{b}}){Adri{\'a}n-Mart{\'{\i}}nez}, {Ageron}, {Albert},
  {Samarai}, {Andr{\'e}}, {Anton}, {Ardid}, {Aubert}, {Baret},
  {Barrios-Mart{\'{\i}}}, {Basa}, {Bertin}, {Biagi}, {Bogazzi}, {Bormuth},
  {Bou-Cabo}, {Bouwhuis}, {Bruijn}, {Brunner}, {Busto}, {Capone}, {Caramete},
  {Carr}, {Chiarusi}, {Circella}, {Coniglione}, {Costantini}, {Coyle},
  {Creusot}, {Dekeyser}, {Deschamps}, {De Bonis}, {Distefano}, {Donzaud},
  {Dornic}, {Drouhin}, {Dumas}, {Eberl}, {Els{\"a}sser}, {Enzenh{\"o}fer},
  {Fehn}, {Felis}, {Fermani}, {Folger}, {Fusco}, {Galat{\`a}}, {Gay},
  {Gei{\ss}els{\"o}der}, {Geyer}, {Giordano}, {Gleixner}, {Gracia-Ruiz},
  {Graf}, {van Haren}, {Heijboer}, {Hello}, {Hern{\'a}ndez-Rey}, {Herrero},
  {H{\"o}{\ss}l}, {Hofest{\"a}dt}, {Hugon}, {James}, {de Jong}, {Kadler},
  {Kalekin}, {Katz}, {Kie{\ss}ling}, {Kooijman}, {Kouchner}, {Kreykenbohm},
  {Kulikovskiy}, {Lahmann}, {Lambard}, {Lattuada}, {Lef{\`e}vre}, {Leonora},
  {Loucatos}, {Mangano}, {Marcelin}, {Margiotta}, {Mart{\'{\i}}nez-Mora},
  {Martini}, {Mathieu}, {Michael}, {Migliozzi}, {Moussa}, {Mueller}, {Neff},
  {Nezri}, {P{\u a}v{\u a}la{\v s}}, {Pellegrino}, {Perrina}, {Piattelli},
  {Popa}, {Pradier}, {Racca}, {Riccobene}, {Richter}, {Roensch}, {Rostovtsev},
  {Salda{\~n}a}, {Samtleben}, {Sanguineti}, {Sapienza}, {Schmid}, {Schnabel},
  {Schulte}, {Sch{\"u}ssler}, {Seitz}, {Sieger}, {Spurio}, {Steijger},
  {Stolarczyk}, {S{\'a}nchez-Losa}, {Taiuti}, {Tamburini}, {Trovato},
  {Tselengidou}, {T{\"o}nnis}, {Turpin}, {Vallage}, {Vall{\'e}e}, {Van
  Elewyck}, {Vecchi}, {Visser}, {Vivolo}, {Wagner}, {Wilms}, {Zornoza},
  {Z{\'u}{\~n}iga}, {Klotz}, {Boer}, {Le Van Suu}, {Akerlof}, {Zheng}, {Evans},
  {Gehrels}, {Kennea}, {Osborne}, \& {Coward}}]{Antares2016}
{Adri{\'a}n-Mart{\'{\i}}nez}, S., {Ageron}, M., {Albert}, A., {et~al.}
  2016{\natexlab{b}}, \jcap, 2, 062

\bibitem[{{Ageron} {et~al.}(2012){Ageron}, {Aguilar}, {Al Samarai}, {Albert},
  {Andr{\'e}}, {Anghinolfi}, {Anton}, {Anvar}, {Ardid}, {Assis Jesus},
  {Astraatmadja}, {Aubert}, {Baret}, {Basa}, {Bertin}, {Biagi}, {Bigi},
  {Bigongiari}, {Bogazzi}, {Bou-Cabo}, {Bouhou}, {Bouwhuis}, {Brunner},
  {Busto}, {Camarena}, {Capone}, {C{\^a}rloganu}, {Carminati}, {Carr},
  {Cecchini}, {Charif}, {Charvis}, {Chiarusi}, {Circella}, {Coniglione},
  {Costantini}, {Coyle}, {Curtil}, {Decowski}, {Dekeyser}, {Deschamps},
  {Distefano}, {Donzaud}, {Dornic}, {Dorosti}, {Drouhin}, {Eberl}, {Emanuele},
  {Enzenh{\"o}fer}, {Ernenwein}, {Escoffier}, {Fermani}, {Ferri}, {Flaminio},
  {Folger}, {Fritsch}, {Fuda}, {Galat{\`a}}, {Gay}, {Giacomelli}, {Giordano},
  {G{\'o}mez-Gonz{\'a}lez}, {Graf}, {Guillard}, {Halladjian}, {Hallewell}, {van
  Haren}, {Hartman}, {Heijboer}, {Hello}, {Hern{\'a}ndez-Rey}, {Herold},
  {H{\"o}{\ss}l}, {Hsu}, {de Jong}, {Kadler}, {Kalekin}, {Kappes}, {Katz},
  {Kavatsyuk}, {Kooijman}, {Kopper}, {Kouchner}, {Kreykenbohm}, {Kulikovskiy},
  {Lahmann}, {Lamare}, {Larosa}, {Lattuada}, {Lef{\`e}vre}, {Lim}, {Lo Presti},
  {Loehner}, {Loucatos}, {Mangano}, {Marcelin}, {Margiotta},
  {Mart{\'{\i}}nez-Mora}, {Meli}, {Montaruli}, {Moscoso}, {Motz}, {Neff},
  {Nezri}, {Palioselitis}, {P{\u a}v{\u a}la{\c s}}, {Payet}, {Payre},
  {Petrovic}, {Piattelli}, {Picot-Clemente}, {Popa}, {Pradier}, {Presani},
  {Racca}, {Reed}, {Richardt}, {Richter}, {Rivi{\`e}re}, {Robert}, {Roensch},
  {Rostovtsev}, {Ruiz-Rivas}, {Rujoiu}, {Russo}, {Salesa}, {Sapienza},
  {Sch{\"o}ck}, {Schuller}, {Sch{\"u}ssler}, {Shanidze}, {Simeone}, {Spies},
  {Spurio}, {Steijger}, {Stolarczyk}, {S{\'a}nchez-Losa}, {Taiuti},
  {Tamburini}, {Toscano}, {Vallage}, {van Elewyck}, {Vannoni}, {Vecchi},
  {Vernin}, {Wijnker}, {Wilms}, {de Wolf}, {Yepes}, {Zaborov}, {Zornoza}, \&
  {Z{\'u}{\~n}iga}}]{Antares2012}
{Ageron}, M., {Aguilar}, J.~A., {Al Samarai}, I., {et~al.} 2012, Astroparticle
  Physics, 35, 530

\bibitem[{{Ajello} {et~al.}(2009){Ajello}, {Costamante}, {Sambruna}, {Gehrels},
  {Chiang}, {Rau}, {Escala}, {Greiner}, {Tueller}, {Wall}, \&
  {Mushotzky}}]{Ajello2009}
{Ajello}, M., {Costamante}, L., {Sambruna}, R.~M., {et~al.} 2009, \apj, 699,
  603

\bibitem[{{Amati}(2006{\natexlab{a}})}]{Amati2006}
{Amati}, L. 2006{\natexlab{a}}, \mnras, 372, 233

\bibitem[{{Amati}(2006{\natexlab{b}})}]{2006MNRAS.372..233A}
---. 2006{\natexlab{b}}, \mnras, 372, 233

\bibitem[{{Amati} {et~al.}(2002){Amati}, {Frontera}, {Tavani}, {in't Zand},
  {Antonelli}, {Costa}, {Feroci}, {Guidorzi}, {Heise}, {Masetti}, {Montanari},
  {Nicastro}, {Palazzi}, {Pian}, {Piro}, \& {Soffitta}}]{2002A&A...390...81A}
{Amati}, L., {Frontera}, F., {Tavani}, M., {et~al.} 2002, \aap, 390, 81

\bibitem[{{Ando} \& {Beacom}(2005)}]{Ando2005}
{Ando}, S., \& {Beacom}, J.~F. 2005, Physical Review Letters, 95, 061103

\bibitem[{{Angel}(1979)}]{angel}
{Angel}, J.~R.~P. 1979, \apj, 233, 364

\bibitem[{{Antier} {et~al.}(2015){Antier}, {Schanne}, {Cordier}, {Gros},
  {G{\"o}tz}, \& {Lachaud}}]{Antier:15}
{Antier}, S., {Schanne}, S., {Cordier}, B., {et~al.} 2015, ArXiv e-prints,
  arXiv:1508.05505

\bibitem[{{Atteia}(2003)}]{2003A&A...407L...1A}
{Atteia}, J.-L. 2003, \aap, 407, L1

\bibitem[{{Bachetti} {et~al.}(2014){Bachetti}, {Harrison}, {Walton},
  {Grefenstette}, {Chakrabarty}, {F{\"u}rst}, {Barret}, {Beloborodov}, {Boggs},
  {Christensen}, {Craig}, {Fabian}, {Hailey}, {Hornschemeier}, {Kaspi},
  {Kulkarni}, {Maccarone}, {Miller}, {Rana}, {Stern}, {Tendulkar}, {Tomsick},
  {Webb}, \& {Zhang}}]{bachetti:14}
{Bachetti}, M., {Harrison}, F.~A., {Walton}, D.~J., {et~al.} 2014, \nat, 514,
  202

\bibitem[{{Band} {et~al.}(1993){Band}, {Matteson}, {Ford}, {Schaefer},
  {Palmer}, {Teegarden}, {Cline}, {Briggs}, {Paciesas}, {Pendleton}, {Fishman},
  {Kouveliotou}, {Meegan}, {Wilson}, \& {Lestrade}}]{1993ApJ...413..281B}
{Band}, D., {Matteson}, J., {Ford}, L., {et~al.} 1993, \apj, 413, 281

\bibitem[{{Barnes} \& {Kasen}(2013)}]{barnes:2013}
{Barnes}, J., \& {Kasen}, D. 2013, \apj, 775, 18

\bibitem[{{Barthelmy} {et~al.}(2005){Barthelmy}, {Barbier}, {Cummings},
  {Fenimore}, {Gehrels}, {Hullinger}, {Krimm}, {Markwardt}, {Palmer},
  {Parsons}, {Sato}, {Suzuki}, {Takahashi}, {Tashiro}, \&
  {Tueller}}]{Barthelmy:05}
{Barthelmy}, S.~D., {Barbier}, L.~M., {Cummings}, J.~R., {et~al.} 2005, \ssr,
  120, 143

\bibitem[{{Basa} {et~al.}(2012){Basa}, {Cuby}, {Savaglio}, {Boissier},
  {Cl{\'e}ment}, {Flores}, {Le Borgne}, \& {Mazure}}]{2012A&A...542A.103B}
{Basa}, S., {Cuby}, J.~G., {Savaglio}, S., {et~al.} 2012, \aap, 542, A103

\bibitem[{{Becker} {et~al.}(2007){Becker}, {Rauch}, \& {Sargent}}]{Becker2007}
{Becker}, G.~D., {Rauch}, M., \& {Sargent}, W.~L.~W. 2007, \apj, 662, 72

\bibitem[{{Beckmann} \& {Shrader}(2012)}]{Beckmann2012}
{Beckmann}, V., \& {Shrader}, C.~R. 2012, {Active Galactic Nuclei}

\bibitem[{{Beloborodov}(2010)}]{beloborodov:10}
{Beloborodov}, A.~M. 2010, \mnras, 407, 1033

\bibitem[{{Berger}(2014)}]{Berger:2014}
{Berger}, E. 2014, \araa, 52, 43

\bibitem[{{Blanchard} {et~al.}(2016){Blanchard}, {Berger}, \&
  {Fong}}]{Blanchard16}
{Blanchard}, P.~K., {Berger}, E., \& {Fong}, W.-f. 2016, \apj, 817, 144

\bibitem[{{Blandford} \& {Znajek}(1977)}]{Bland1977}
{Blandford}, R.~D., \& {Znajek}, R.~L. 1977, \mnras, 179, 433

\bibitem[{{Bloom} {et~al.}(2008){Bloom}, {Butler}, \& {Perley}}]{bloom:2008}
{Bloom}, J.~S., {Butler}, N.~R., \& {Perley}, D.~A. 2008, in American Institute
  of Physics Conference Series, Vol. 1000, American Institute of Physics
  Conference Series, ed. M.~{Galassi}, D.~{Palmer}, \& E.~{Fenimore}, 11--15

\bibitem[{{Bloom} {et~al.}(2003){Bloom}, {Frail}, \&
  {Kulkarni}}]{2003ApJ...594..674B}
{Bloom}, J.~S., {Frail}, D.~A., \& {Kulkarni}, S.~R. 2003, \apj, 594, 674

\bibitem[{{Bloom} {et~al.}(2009){Bloom}, {Holz}, {Hughes}, {Menou}, {Adams},
  {Anderson}, {Becker}, {Bower}, {Brandt}, {Cobb}, {Cook}, {Corsi}, {Covino},
  {Fox}, {Fruchter}, {Fryer}, {Grindlay}, {Hartmann}, {Haiman}, {Kocsis},
  {Jones}, {Loeb}, {Marka}, {Metzger}, {Nakar}, {Nissanke}, {Perley}, {Piran},
  {Poznanski}, {Prince}, {Schnittman}, {Soderberg}, {Strauss}, {Shawhan},
  {Shoemaker}, {Sievers}, {Stubbs}, {Tagliaferri}, {Ubertini}, \&
  {Wozniak}}]{bloom:2009}
{Bloom}, J.~S., {Holz}, D.~E., {Hughes}, S.~A., {et~al.} 2009, ArXiv e-prints,
  arXiv:0902.1527

\bibitem[{{Bode}(2015)}]{ASTRONET:FP7}
{Bode}, M. 2015, ASTRONET, \url{http://www.astronet-eu.org}

\bibitem[{{Boissier} {et~al.}(2013){Boissier}, {Salvaterra}, {Le Floc'h},
  {Basa}, {Buat}, {Prantzos}, {Vergani}, \& {Savaglio}}]{boissier13}
{Boissier}, S., {Salvaterra}, R., {Le Floc'h}, E., {et~al.} 2013, \aap, 557,
  A34

\bibitem[{{Bournaud} {et~al.}(2014){Bournaud}, {Perret}, {Renaud}, {Dekel},
  {Elmegreen}, {Elmegreen}, {Teyssier}, {Amram}, {Daddi}, {Duc}, {Elbaz},
  {Epinat}, {Gabor}, {Juneau}, {Kraljic}, \& {Le Floch'}}]{Bournaud14}
{Bournaud}, F., {Perret}, V., {Renaud}, F., {et~al.} 2014, \apj, 780, 57

\bibitem[{{Bouwens} {et~al.}(2009){Bouwens}, {Illingworth}, {Franx}, {Chary},
  {Meurer}, {Conselice}, {Ford}, {Giavalisco}, \& {van Dokkum}}]{Bouwens2009}
{Bouwens}, R.~J., {Illingworth}, G.~D., {Franx}, M., {et~al.} 2009, \apj, 705,
  936

\bibitem[{{Bouwens} {et~al.}(2011){Bouwens}, {Illingworth}, {Labbe}, {Oesch},
  {Trenti}, {Carollo}, {van Dokkum}, {Franx}, {Stiavelli}, {Gonz{\'a}lez},
  {Magee}, \& {Bradley}}]{Bouwens2011}
{Bouwens}, R.~J., {Illingworth}, G.~D., {Labbe}, I., {et~al.} 2011, \nat, 469,
  504

\bibitem[{{Bouwens} {et~al.}(2015){Bouwens}, {Illingworth}, {Oesch}, {Trenti},
  {Labb{\'e}}, {Bradley}, {Carollo}, {van Dokkum}, {Gonzalez}, {Holwerda},
  {Franx}, {Spitler}, {Smit}, \& {Magee}}]{2015ApJ...803...34B}
{Bouwens}, R.~J., {Illingworth}, G.~D., {Oesch}, P.~A., {et~al.} 2015, \apj,
  803, 34

\bibitem[{{Bromberg} {et~al.}(2011){Bromberg}, {Nakar}, \&
  {Piran}}]{bromberg:2011}
{Bromberg}, O., {Nakar}, E., \& {Piran}, T. 2011, \apjl, 739, L55

\bibitem[{{Bromberg} {et~al.}(2013){Bromberg}, {Nakar}, {Piran}, \&
  {Sari}}]{bromberg:2013}
{Bromberg}, O., {Nakar}, E., {Piran}, T., \& {Sari}, R. 2013, \apj, 764, 179

\bibitem[{{Bromm} {et~al.}(2002){Bromm}, {Coppi}, \& {Larson}}]{Bromm2002}
{Bromm}, V., {Coppi}, P.~S., \& {Larson}, R.~B. 2002, \apj, 564, 23

\bibitem[{{Bromm} \& {Loeb}(2006)}]{2006ApJ...642..382B}
{Bromm}, V., \& {Loeb}, A. 2006, \apj, 642, 382

\bibitem[{{Bucciantini} {et~al.}(2009){Bucciantini}, {Quataert}, {Metzger},
  {Thompson}, {Arons}, \& {Del Zanna}}]{Bucc2009}
{Bucciantini}, N., {Quataert}, E., {Metzger}, B.~D., {et~al.} 2009, \mnras,
  396, 2038

\bibitem[{{Butler} {et~al.}(2007){Butler}, {Kocevski}, {Bloom}, \&
  {Curtis}}]{2007ApJ...671..656B}
{Butler}, N.~R., {Kocevski}, D., {Bloom}, J.~S., \& {Curtis}, J.~L. 2007, \apj,
  671, 656

\bibitem[{{Campana} {et~al.}(2011){Campana}, {Lodato}, {D'Avanzo}, {Panagia},
  {Rossi}, {Della Valle}, {Tagliaferri}, {Antonelli}, {Covino}, {Ghirlanda},
  {Ghisellini}, {Melandri}, {Pian}, {Salvaterra}, {Cusumano}, {D'Elia},
  {Fugazza}, {Palazzi}, {Sbarufatti}, \& {Vergani}}]{campana:2011}
{Campana}, S., {Lodato}, G., {D'Avanzo}, P., {et~al.} 2011, \nat, 480, 69

\bibitem[{{Cano} {et~al.}(2016){Cano}, {Wang}, {Dai}, \& {Wu}}]{Cano2016}
{Cano}, Z., {Wang}, S.-Q., {Dai}, Z.-G., \& {Wu}, X.-F. 2016, ArXiv:1604.03549,
  arXiv:1604.03549

\bibitem[{{Castro-Tirado} {et~al.}(2010){Castro-Tirado}, {M{\o}ller},
  {Garc{\'{\i}}a-Segura}, {Gorosabel}, {P{\'e}rez}, {de Ugarte Postigo},
  {Solano}, {Barrado}, {Klose}, {Kann}, {Castro Cer{\'o}n}, {Kouveliotou},
  {Fynbo}, {Hjorth}, {Pedersen}, {Pian}, {Rol}, {Palazzi}, {Masetti}, {Tanvir},
  {Vreeswijk}, {Andersen}, {Fruchter}, {Greiner}, {Wijers}, \& {van den
  Heuvel}}]{castrotirado2010}
{Castro-Tirado}, A.~J., {M{\o}ller}, P., {Garc{\'{\i}}a-Segura}, G., {et~al.}
  2010, \aap, 517, A61

\bibitem[{{Chen} {et~al.}(2007){Chen}, {Prochaska}, \&
  {Gnedin}}]{2007ApJ...667L.125C}
{Chen}, H.-W., {Prochaska}, J.~X., \& {Gnedin}, N.~Y. 2007, \apjl, 667, L125

\bibitem[{{Cheng} {et~al.}(2010){Cheng}, {Yu}, \& {Harko}}]{Cheng2010}
{Cheng}, K.~S., {Yu}, Y.-W., \& {Harko}, T. 2010, Physical Review Letters, 104,
  241102

\bibitem[{{Chornock} {et~al.}(2014){Chornock}, {Berger}, {Fox}, {Fong},
  {Laskar}, \& {Roth}}]{2014arXiv1405.7400C}
{Chornock}, R., {Berger}, E., {Fox}, D.~B., {et~al.} 2014, ArXiv e-prints,
  arXiv:1405.7400

\bibitem[{{Christensen} {et~al.}(2008){Christensen}, {Vreeswijk}, {Sollerman},
  {Th{\"o}ne}, {Le Floc'h}, \& {Wiersema}}]{Christensen08}
{Christensen}, L., {Vreeswijk}, P.~M., {Sollerman}, J., {et~al.} 2008, \aap,
  490, 45

\bibitem[{{Chu} {et~al.}(2016){Chu}, {Howell}, {Rowlinson}, {Gao}, {Zhang},
  {Tingay}, {Bo{\"e}r}, \& {Wen}}]{chu16}
{Chu}, Q., {Howell}, E.~J., {Rowlinson}, A., {et~al.} 2016, \mnras, 459, 121

\bibitem[{{Churazov} {et~al.}(2007){Churazov}, {Sunyaev}, {Revnivtsev},
  {Sazonov}, {Molkov}, {Grebenev}, {Winkler}, {Parmar}, {Bazzano}, {Falanga},
  {Gros}, {Lebrun}, {Natalucci}, {Ubertini}, {Roques}, {Bouchet}, {Jourdain},
  {Kn{\"o}dlseder}, {Diehl}, {Budtz-Jorgensen}, {Brandt}, {Lund},
  {Westergaard}, {Neronov}, {T{\"u}rler}, {Chernyakova}, {Walter}, {Produit},
  {Mowlavi}, {Mas-Hesse}, {Domingo}, {Gehrels}, {Kuulkers}, {Kretschmar}, \&
  {Schmidt}}]{2007A&A...467..529C}
{Churazov}, E., {Sunyaev}, R., {Revnivtsev}, M., {et~al.} 2007, \aap, 467, 529

\bibitem[{{Committee for a Decadal Survey of Astronomy and
  Astrophysics}(2010)}]{decadal:2010}
{Committee for a Decadal Survey of Astronomy and Astrophysics}. 2010, National
  Academies Press

\bibitem[{Connaughton {et~al.}(2015)}]{Connaughton:2014xha}
Connaughton, V., {et~al.} 2015, Astrophys. J. Suppl., 216, 32

\bibitem[{{Corbel} {et~al.}(2003){Corbel}, {Nowak}, {Fender}, {Tzioumis}, \&
  {Markoff}}]{corbel03}
{Corbel}, S., {Nowak}, M.~A., {Fender}, R.~P., {Tzioumis}, A.~K., \& {Markoff},
  S. 2003, \aap, 400, 1007

\bibitem[{{Cordier} {et~al.}(2008){Cordier}, {Desclaux}, {Foliard}, \&
  {Schanne}}]{cord}
{Cordier}, B., {Desclaux}, F., {Foliard}, J., \& {Schanne}, S. 2008, in
  American Institute of Physics Conference Series, Vol. 1000, American
  Institute of Physics Conference Series, ed. M.~{Galassi}, D.~{Palmer}, \&
  E.~{Fenimore}, 585--588

\bibitem[{{Cordier} {et~al.}(2015){Cordier}, {Wei}, {Atteia}, {Basa}, {Claret},
  {Daigne}, {Deng}, {Dong}, {Godet}, {Goldwurm}, {G{\"o}tz}, {Han}, {Klotz},
  {Lachaud}, {Osborne}, {Qiu}, {Schanne}, {Wu}, {Wang}, {Wu}, {Xin}, {Zhang},
  \& {Zhang}}]{2015arXiv151203323C}
{Cordier}, B., {Wei}, J., {Atteia}, J.-L., {et~al.} 2015, ArXiv e-prints,
  arXiv:1512.03323

\bibitem[{{Coriat} {et~al.}(2011){Coriat}, {Corbel}, {Prat}, {Miller-Jones},
  {Cseh}, {Tzioumis}, {Brocksopp}, {Rodriguez}, {Fender}, \&
  {Sivakoff}}]{mickael_1743}
{Coriat}, M., {Corbel}, S., {Prat}, L., {et~al.} 2011, \mnras, 414, 677

\bibitem[{{Coward}(2007)}]{Coward2007}
{Coward}, D. 2007, NewAR, 51, 539

\bibitem[{{Dai} {et~al.}(2006){Dai}, {Wang}, {Wu}, \& {Zhang}}]{Dai2006}
{Dai}, Z.~G., {Wang}, X.~Y., {Wu}, X.~F., \& {Zhang}, B. 2006, Science, 311,
  1127

\bibitem[{{Daigne} \& {Mochkovitch}(1998)}]{daigne:98}
{Daigne}, F., \& {Mochkovitch}, R. 1998, \mnras, 296, 275

\bibitem[{{Daigne} \& {Mochkovitch}(2002)}]{daigne:02}
---. 2002, \mnras, 336, 1271

\bibitem[{{Daigne} {et~al.}(2006{\natexlab{a}}){Daigne}, {Rossi}, \&
  {Mochkovitch}}]{daigne2006}
{Daigne}, F., {Rossi}, E.~M., \& {Mochkovitch}, R. 2006{\natexlab{a}}, \mnras,
  372, 1034

\bibitem[{{Daigne} {et~al.}(2006{\natexlab{b}}){Daigne}, {Rossi}, \&
  {Mochkovitch}}]{daigne06}
---. 2006{\natexlab{b}}, \mnras, 372, 1034

\bibitem[{{Dall'Osso} {et~al.}(2015){Dall'Osso}, {Giacomazzo}, {Perna}, \&
  {Stella}}]{dallosso:2015}
{Dall'Osso}, S., {Giacomazzo}, B., {Perna}, R., \& {Stella}, L. 2015, \apj,
  798, 25

\bibitem[{{De Cia} {et~al.}(2012){De Cia}, {Ledoux}, {Fox}, {Vreeswijk},
  {Smette}, {Petitjean}, {Bj{\"o}rnsson}, {Fynbo}, {Hjorth}, \&
  {Jakobsson}}]{Cia2012}
{De Cia}, A., {Ledoux}, C., {Fox}, A.~J., {et~al.} 2012, \aap, 545, A64

\bibitem[{{Di Sciascio} \& {on behalf of the LHAASO
  Collaboration}(2016)}]{DiSciascio2016}
{Di Sciascio}, G., \& {on behalf of the LHAASO Collaboration}. 2016, ArXiv
  e-prints, arXiv:1602.07600

\bibitem[{{Elliott} {et~al.}(2012){Elliott}, {Greiner}, {Khochfar}, {Schady},
  {Johnson}, \& {Rau}}]{elliott12}
{Elliott}, J., {Greiner}, J., {Khochfar}, S., {et~al.} 2012, \aap, 539, A113

\bibitem[{{Evans} {et~al.}(2007){Evans}, {Beardmore}, {Page}, {Tyler},
  {Osborne}, {Goad}, {O'Brien}, {Vetere}, {Racusin}, {Morris}, {Burrows},
  {Capalbi}, {Perri}, {Gehrels}, \& {Romano}}]{evans:2007}
{Evans}, P.~A., {Beardmore}, A.~P., {Page}, K.~L., {et~al.} 2007, \aap, 469,
  379

\bibitem[{{Evans} {et~al.}(2009){Evans}, {Beardmore}, {Page}, {Osborne},
  {O'Brien}, {Willingale}, {Starling}, {Burrows}, {Godet}, {Vetere}, {Racusin},
  {Goad}, {Wiersema}, {Angelini}, {Capalbi}, {Chincarini}, {Gehrels}, {Kennea},
  {Margutti}, {Morris}, {Mountford}, {Pagani}, {Perri}, {Romano}, \&
  {Tanvir}}]{evans:2009}
---. 2009, \mnras, 397, 1177

\bibitem[{{Evans} {et~al.}(2016){Evans}, {Osborne}, {Kennea}, {Campana},
  {O'Brien}, {Tanvir}, {Racusin}, {Burrows}, {Cenko}, \&
  {Gehrels}}]{evans:2016}
{Evans}, P.~A., {Osborne}, J.~P., {Kennea}, J.~A., {et~al.} 2016, \mnras, 455,
  1522

\bibitem[{{Fabbiano}(1989)}]{fabbiano:89}
{Fabbiano}, G. 1989, \araa, 27, 87

\bibitem[{{Fabian} \& {Iwasawa}(1999)}]{1999MNRAS.303L..34F}
{Fabian}, A.~C., \& {Iwasawa}, K. 1999, \mnras, 303, L34

\bibitem[{{Fan} \& {Xu}(2006)}]{fan:2006}
{Fan}, Y.-Z., \& {Xu}, D. 2006, \mnras, 372, L19

\bibitem[{{Fern{\'a}ndez} \& {Metzger}(2015)}]{fernandez:2015}
{Fern{\'a}ndez}, R., \& {Metzger}, B.~D. 2015, ArXiv e-prints, arXiv:1512.05435

\bibitem[{{Firmani} {et~al.}(2006){Firmani}, {Ghisellini}, {Avila-Reese}, \&
  {Ghirlanda}}]{2006MNRAS.370..185F}
{Firmani}, C., {Ghisellini}, G., {Avila-Reese}, V., \& {Ghirlanda}, G. 2006,
  \mnras, 370, 185

\bibitem[{{Fox} {et~al.}(2008){Fox}, {Ledoux}, {Vreeswijk}, {Smette}, \&
  {Jaunsen}}]{fox2008}
{Fox}, A.~J., {Ledoux}, C., {Vreeswijk}, P.~M., {Smette}, A., \& {Jaunsen},
  A.~O. 2008, \aap, 491, 189

\bibitem[{{Frail} {et~al.}(2001){Frail}, {Kulkarni}, {Sari}, {Djorgovski},
  {Bloom}, {Galama}, {Reichart}, {Berger}, {Harrison}, {Price}, {Yost},
  {Diercks}, {Goodrich}, \& {Chaffee}}]{2001ApJ...562L..55F}
{Frail}, D.~A., {Kulkarni}, S.~R., {Sari}, R., {et~al.} 2001, \apjl, 562, L55

\bibitem[{{Fruchter} {et~al.}(2006){Fruchter}, {Levan}, {Strolger},
  {Vreeswijk}, {Thorsett}, {Bersier}, {Burud}, {Castro Cer{\'o}n},
  {Castro-Tirado}, {Conselice}, {Dahlen}, {Ferguson}, {Fynbo}, {Garnavich},
  {Gibbons}, {Gorosabel}, {Gull}, {Hjorth}, {Holland}, {Kouveliotou}, {Levay},
  {Livio}, {Metzger}, {Nugent}, {Petro}, {Pian}, {Rhoads}, {Riess}, {Sahu},
  {Smette}, {Tanvir}, {Wijers}, \& {Woosley}}]{Fruchter06}
{Fruchter}, A.~S., {Levan}, A.~J., {Strolger}, L., {et~al.} 2006, \nat, 441,
  463

\bibitem[{{Fryer} {et~al.}(2015){Fryer}, {Belczynski}, {Ramirez-Ruiz},
  {Rosswog}, {Shen}, \& {Steiner}}]{fryer:2015}
{Fryer}, C.~L., {Belczynski}, K., {Ramirez-Ruiz}, E., {et~al.} 2015, \apj, 812,
  24

\bibitem[{Fryer \& New(2011)}]{FryerLRR}
Fryer, C.~L., \& New, K.~C. 2011, Living Reviews in Relativity, 14,
  doi:10.1007/lrr-2011-1

\bibitem[{{Fynbo} {et~al.}(2006){Fynbo}, {Watson}, {Th{\"o}ne}, {Sollerman},
  {Bloom}, {Davis}, {Hjorth}, {Jakobsson}, {J{\o}rgensen}, {Graham},
  {Fruchter}, {Bersier}, {Kewley}, {Cassan}, {Castro Cer{\'o}n}, {Foley},
  {Gorosabel}, {Hinse}, {Horne}, {Jensen}, {Klose}, {Kocevski}, {Marquette},
  {Perley}, {Ramirez-Ruiz}, {Stritzinger}, {Vreeswijk}, {Wijers}, {Woller},
  {Xu}, \& {Zub}}]{Fynbo2006}
{Fynbo}, J.~P.~U., {Watson}, D., {Th{\"o}ne}, C.~C., {et~al.} 2006, \nat, 444,
  1047

\bibitem[{{Fynbo} {et~al.}(2009){Fynbo}, {Jakobsson}, {Prochaska}, {Malesani},
  {Ledoux}, {de Ugarte Postigo}, {Nardini}, {Vreeswijk}, {Wiersema}, {Hjorth},
  {Sollerman}, {Chen}, {Th{\"o}ne}, {Bj{\"o}rnsson}, {Bloom}, {Castro-Tirado},
  {Christensen}, {De Cia}, {Fruchter}, {Gorosabel}, {Graham}, {Jaunsen},
  {Jensen}, {Kann}, {Kouveliotou}, {Levan}, {Maund}, {Masetti},
  {Milvang-Jensen}, {Palazzi}, {Perley}, {Pian}, {Rol}, {Schady}, {Starling},
  {Tanvir}, {Watson}, {Xu}, {Augusteijn}, {Grundahl}, {Telting}, \&
  {Quirion}}]{2009ApJS..185..526F}
{Fynbo}, J.~P.~U., {Jakobsson}, P., {Prochaska}, J.~X., {et~al.} 2009, \apjs,
  185, 526

\bibitem[{{Gal-Yam} {et~al.}(2006){Gal-Yam}, {Fox}, {Price}, {Ofek}, {Davis},
  {Leonard}, {Soderberg}, {Schmidt}, {Lewis}, {Peterson}, {Kulkarni}, {Berger},
  {Cenko}, {Sari}, {Sharon}, {Frail}, {Moon}, {Brown}, {Cucchiara}, {Harrison},
  {Piran}, {Persson}, {McCarthy}, {Penprase}, {Chevalier}, \&
  {MacFadyen}}]{galyam:2006}
{Gal-Yam}, A., {Fox}, D.~B., {Price}, P.~A., {et~al.} 2006, \nat, 444, 1053

\bibitem[{{Gao} {et~al.}(2015){Gao}, {Ding}, {Wu}, {Dai}, \& {Zhang}}]{Gao15}
{Gao}, H., {Ding}, X., {Wu}, X.-F., {Dai}, Z.-G., \& {Zhang}, B. 2015, \apj,
  807, 163

\bibitem[{{Gehrels} {et~al.}(2016){Gehrels}, {Cannizzo}, {Kanner}, {Kasliwal},
  {Nissanke}, \& {Singer}}]{gehrels:2016}
{Gehrels}, N., {Cannizzo}, J.~K., {Kanner}, J., {et~al.} 2016, \apj, 820, 136

\bibitem[{{Gehrels} \& {Razzaque}(2013)}]{gehrels:13}
{Gehrels}, N., \& {Razzaque}, S. 2013, Frontiers of Physics, 8, 661

\bibitem[{{Gehrels} {et~al.}(2004){Gehrels}, {Chincarini}, {Giommi}, {Mason},
  {Nousek}, {Wells}, {White}, {Barthelmy}, {Burrows}, {Cominsky}, {Hurley},
  {Marshall}, {M{\'e}sz{\'a}ros}, {Roming}, {Angelini}, {Barbier}, {Belloni},
  {Campana}, {Caraveo}, {Chester}, {Citterio}, {Cline}, {Cropper}, {Cummings},
  {Dean}, {Feigelson}, {Fenimore}, {Frail}, {Fruchter}, {Garmire}, {Gendreau},
  {Ghisellini}, {Greiner}, {Hill}, {Hunsberger}, {Krimm}, {Kulkarni}, {Kumar},
  {Lebrun}, {Lloyd-Ronning}, {Markwardt}, {Mattson}, {Mushotzky}, {Norris},
  {Osborne}, {Paczynski}, {Palmer}, {Park}, {Parsons}, {Paul}, {Rees},
  {Reynolds}, {Rhoads}, {Sasseen}, {Schaefer}, {Short}, {Smale}, {Smith},
  {Stella}, {Tagliaferri}, {Takahashi}, {Tashiro}, {Townsley}, {Tueller},
  {Turner}, {Vietri}, {Voges}, {Ward}, {Willingale}, {Zerbi}, \&
  {Zhang}}]{gehrels:2004}
{Gehrels}, N., {Chincarini}, G., {Giommi}, P., {et~al.} 2004, \apj, 611, 1005

\bibitem[{{Gehrels} {et~al.}(2005){Gehrels}, {Sarazin}, {O'Brien}, {Zhang},
  {Barbier}, {Barthelmy}, {Blustin}, {Burrows}, {Cannizzo}, {Cummings}, {Goad},
  {Holland}, {Hurkett}, {Kennea}, {Levan}, {Markwardt}, {Mason}, {Meszaros},
  {Page}, {Palmer}, {Rol}, {Sakamoto}, {Willingale}, {Angelini}, {Beardmore},
  {Boyd}, {Breeveld}, {Campana}, {Chester}, {Chincarini}, {Cominsky},
  {Cusumano}, {de Pasquale}, {Fenimore}, {Giommi}, {Gronwall}, {Grupe}, {Hill},
  {Hinshaw}, {Hjorth}, {Hullinger}, {Hurley}, {Klose}, {Kobayashi},
  {Kouveliotou}, {Krimm}, {Mangano}, {Marshall}, {McGowan}, {Moretti},
  {Mushotzky}, {Nakazawa}, {Norris}, {Nousek}, {Osborne}, {Page}, {Parsons},
  {Patel}, {Perri}, {Poole}, {Romano}, {Roming}, {Rosen}, {Sato}, {Schady},
  {Smale}, {Sollerman}, {Starling}, {Still}, {Suzuki}, {Tagliaferri},
  {Takahashi}, {Tashiro}, {Tueller}, {Wells}, {White}, \&
  {Wijers}}]{gehrels:2005}
{Gehrels}, N., {Sarazin}, C.~L., {O'Brien}, P.~T., {et~al.} 2005, \nat, 437,
  851

\bibitem[{{Gendre} {et~al.}(2013){Gendre}, {Stratta}, {Atteia}, {Basa},
  {Bo{\"e}r}, {Coward}, {Cutini}, {D'Elia}, {Howell}, {Klotz}, \&
  {Piro}}]{gendre:2013}
{Gendre}, B., {Stratta}, G., {Atteia}, J.~L., {et~al.} 2013, \apj, 766, 30

\bibitem[{{Ghirlanda} {et~al.}(2015{\natexlab{a}}){Ghirlanda}, {Bernardini},
  {Calderone}, \& {D'Avanzo}}]{ghirlanda:2015}
{Ghirlanda}, G., {Bernardini}, M.~G., {Calderone}, G., \& {D'Avanzo}, P.
  2015{\natexlab{a}}, Journal of High Energy Astrophysics, 7, 81

\bibitem[{{Ghirlanda} {et~al.}(2003){Ghirlanda}, {Celotti}, \&
  {Ghisellini}}]{2003A&A...406..879G}
{Ghirlanda}, G., {Celotti}, A., \& {Ghisellini}, G. 2003, \aap, 406, 879

\bibitem[{{Ghirlanda} {et~al.}(2006){Ghirlanda}, {Ghisellini}, \&
  {Firmani}}]{2006NJPh....8..123G}
{Ghirlanda}, G., {Ghisellini}, G., \& {Firmani}, C. 2006, New Journal of
  Physics, 8, 123

\bibitem[{{Ghirlanda} {et~al.}(2004{\natexlab{a}}){Ghirlanda}, {Ghisellini}, \&
  {Lazzati}}]{2004ApJ...616..331G}
{Ghirlanda}, G., {Ghisellini}, G., \& {Lazzati}, D. 2004{\natexlab{a}}, \apj,
  616, 331

\bibitem[{{Ghirlanda} {et~al.}(2004{\natexlab{b}}){Ghirlanda}, {Ghisellini}, \&
  {Lazzati}}]{Ghirla2004}
---. 2004{\natexlab{b}}, \apj, 616, 331

\bibitem[{{Ghirlanda} {et~al.}(2015{\natexlab{b}}){Ghirlanda}, {Salvaterra},
  {Ghisellini}, {Mereghetti}, {Tagliaferri}, {Campana}, {Osborne}, {O'Brien},
  {Tanvir}, {Willingale}, {Amati}, {Basa}, {Bernardini}, {Burlon}, {Covino},
  {D'Avanzo}, {Frontera}, {G{\"o}tz}, {Melandri}, {Nava}, {Piro}, \&
  {Vergani}}]{2015MNRAS.448.2514G}
{Ghirlanda}, G., {Salvaterra}, R., {Ghisellini}, G., {et~al.}
  2015{\natexlab{b}}, \mnras, 448, 2514

\bibitem[{{Ghisellini} {et~al.}(2015){Ghisellini}, {Tagliaferri}, {Sbarrato},
  \& {Gehrels}}]{Ghisellini2015}
{Ghisellini}, G., {Tagliaferri}, G., {Sbarrato}, T., \& {Gehrels}, N. 2015,
  \mnras, 450, L34

\bibitem[{{Gilmore} {et~al.}(2013){Gilmore}, {Bouvier}, {Connaughton},
  {Goldstein}, {Otte}, {Primack}, \& {Williams}}]{Gilmore2013}
{Gilmore}, R.~C., {Bouvier}, A., {Connaughton}, V., {et~al.} 2013, Experimental
  Astronomy, 35, 413

\bibitem[{{Godet} {et~al.}(2014{\natexlab{a}}){Godet}, {Nasser}, {Atteia},
  {Cordier}, {Mandrou}, {Barret}, {Triou}, {Pons}, {Amoros}, {Bordon}, {Gevin},
  {Gonzalez}, {G{\"o}tz}, {Gros}, {Houret}, {Lachaud}, {Lacombe}, {Marty},
  {Mercier}, {Rambaud}, {Ramon}, {Rouaix}, {Schanne}, \&
  {Waegebaert}}]{Godet:14}
{Godet}, O., {Nasser}, G., {Atteia}, J.-., {et~al.} 2014{\natexlab{a}}, in
  Proc. SPIE, Vol. 9144, Space Telescopes and Instrumentation 2014: Ultraviolet
  to Gamma Ray, 914424

\bibitem[{{Godet} {et~al.}(2014{\natexlab{b}}){Godet}, {Nasser}, {Atteia},
  {Cordier}, {Mandrou}, {Barret}, {Triou}, {Pons}, {Amoros}, {Bordon}, {Gevin},
  {Gonzalez}, {G{\"o}tz}, {Gros}, {Houret}, {Lachaud}, {Lacombe}, {Marty},
  {Mercier}, {Rambaud}, {Ramon}, {Rouaix}, {Schanne}, \&
  {Waegebaert}}]{2014SPIE.9144E..24G}
{Godet}, O., {Nasser}, G., {Atteia}, J.-., {et~al.} 2014{\natexlab{b}}, in
  Proceedings of the SPIE, Vol. 9144, Space Telescopes and Instrumentation
  2014: Ultraviolet to Gamma Ray, 914424

\bibitem[{{Goldstein} {et~al.}(2013){Goldstein}, {Preece}, {Mallozzi},
  {Briggs}, {Fishman}, {Kouveliotou}, {Paciesas}, \&
  {Burgess}}]{goldstein:2013}
{Goldstein}, A., {Preece}, R.~D., {Mallozzi}, R.~S., {et~al.} 2013, \apjs, 208,
  21

\bibitem[{{Goldstein} {et~al.}(2012){Goldstein}, {Burgess}, {Preece}, {Briggs},
  {Guiriec}, {van der Horst}, {Connaughton}, {Wilson-Hodge}, {Paciesas},
  {Meegan}, {von Kienlin}, {Bhat}, {Bissaldi}, {Chaplin}, {Diehl}, {Fishman},
  {Fitzpatrick}, {Foley}, {Gibby}, {Giles}, {Greiner}, {Gruber}, {Kippen},
  {Kouveliotou}, {McBreen}, {McGlynn}, {Rau}, \&
  {Tierney}}]{2012ApJS..199...19G}
{Goldstein}, A., {Burgess}, J.~M., {Preece}, R.~D., {et~al.} 2012, \apjs, 199,
  19

\bibitem[{{Gompertz} {et~al.}(2014){Gompertz}, {O'Brien}, \&
  {Wynn}}]{gompertz:2014}
{Gompertz}, B.~P., {O'Brien}, P.~T., \& {Wynn}, G.~A. 2014, \mnras, 438, 240

\bibitem[{{G{\"o}tz} {et~al.}(2014){G{\"o}tz}, {Osborne}, {Cordier}, {Paul},
  {Evans}, {Beardmore}, {Martindale}, {Willingale}, {O'Brien}, {Basa},
  {Rossin}, {Godet}, {Webb}, {Greiner}, {Nandra}, {Meidinger}, {Perinati},
  {Santangelo}, {Mercier}, \& {Gonzalez}}]{mxt-spie}
{G{\"o}tz}, D., {Osborne}, J., {Cordier}, B., {et~al.} 2014, in Proc. SPIE,
  Vol. 9144, Space Telescopes and Instrumentation 2014: Ultraviolet to Gamma
  Ray, 914423

\bibitem[{{Graham} {et~al.}(2009){Graham}, {Fruchter}, {Kewley}, {Levesque},
  {Levan}, {Tanvir}, {Reichart}, \& {Nysewander}}]{Graham2009}
{Graham}, J.~F., {Fruchter}, A.~S., {Kewley}, L.~J., {et~al.} 2009, in American
  Institute of Physics Conference Series, Vol. 1133, American Institute of
  Physics Conference Series, ed. C.~{Meegan}, C.~{Kouveliotou}, \&
  N.~{Gehrels}, 269--272

\bibitem[{{Granot}(2003)}]{granot:03}
{Granot}, J. 2003, \apjl, 596, L17

\bibitem[{{Greiner} {et~al.}(2015){Greiner}, {Fox}, {Schady}, {Kr{\"u}hler},
  {Trenti}, {Cikota}, {Bolmer}, {Elliott}, {Delvaux}, {Perna}, {Afonso},
  {Kann}, {Klose}, {Savaglio}, {Schmidl}, {Schweyer}, {Tanga}, \&
  {Varela}}]{greiner15}
{Greiner}, J., {Fox}, D.~B., {Schady}, P., {et~al.} 2015, \apj, 809, 76

\bibitem[{{Gruber} {et~al.}(2014{\natexlab{a}}){Gruber}, {Goldstein}, {Weller
  von Ahlefeld}, {Narayana Bhat}, {Bissaldi}, {Briggs}, {Byrne}, {Cleveland},
  {Connaughton}, {Diehl}, {Fishman}, {Fitzpatrick}, {Foley}, {Gibby}, {Giles},
  {Greiner}, {Guiriec}, {van der Horst}, {von Kienlin}, {Kouveliotou},
  {Layden}, {Lin}, {Meegan}, {McGlynn}, {Paciesas}, {Pelassa}, {Preece}, {Rau},
  {Wilson-Hodge}, {Xiong}, {Younes}, \& {Yu}}]{2014ApJS..211...12G}
{Gruber}, D., {Goldstein}, A., {Weller von Ahlefeld}, V., {et~al.}
  2014{\natexlab{a}}, \apjs, 211, 12

\bibitem[{{Gruber} {et~al.}(2014{\natexlab{b}}){Gruber}, {Goldstein}, {Weller
  von Ahlefeld}, {Narayana Bhat}, {Bissaldi}, {Briggs}, {Byrne}, {Cleveland},
  {Connaughton}, {Diehl}, {Fishman}, {Fitzpatrick}, {Foley}, {Gibby}, {Giles},
  {Greiner}, {Guiriec}, {van der Horst}, {von Kienlin}, {Kouveliotou},
  {Layden}, {Lin}, {Meegan}, {McGlynn}, {Paciesas}, {Pelassa}, {Preece}, {Rau},
  {Wilson-Hodge}, {Xiong}, {Younes}, \& {Yu}}]{gruber:2014}
---. 2014{\natexlab{b}}, \apjs, 211, 12

\bibitem[{{Guaita} {et~al.}(2016){Guaita}, {Pentericci}, {Grazian}, {Vanzella},
  {Nonino}, {Giavalisco}, {Zamorani}, {Bongiorno}, {Cassata}, {Castellano},
  {Garilli}, {Gawiser}, {Le Brun}, {Le F{\`e}vre}, {Lemaux}, {Maccagni},
  {Merlin}, {Santini}, {Tasca}, {Thomas}, {Zucca}, {De Barros}, {Hathi},
  {Amorin}, {Bardelli}, \& {Fontana}}]{2016A&A...587A.133G}
{Guaita}, L., {Pentericci}, L., {Grazian}, A., {et~al.} 2016, \aap, 587, A133

\bibitem[{{Guimar{\~a}es} {et~al.}(2007){Guimar{\~a}es}, {Petitjean},
  {Rollinde}, {de Carvalho}, {Djorgovski}, {Srianand}, {Aghaee}, \&
  {Castro}}]{Guimaraes2007}
{Guimar{\~a}es}, R., {Petitjean}, P., {Rollinde}, E., {et~al.} 2007, \mnras,
  377, 657

\bibitem[{{Guiriec} {et~al.}(2010{\natexlab{a}}){Guiriec}, {Briggs},
  {Connaugthon}, {Kara}, {Daigne}, {Kouveliotou}, {van der Horst}, {Paciesas},
  {Meegan}, {Bhat}, {Foley}, {Bissaldi}, {Burgess}, {Chaplin}, {Diehl},
  {Fishman}, {Gibby}, {Giles}, {Goldstein}, {Greiner}, {Gruber}, {von Kienlin},
  {Kippen}, {McBreen}, {Preece}, {Rau}, {Tierney}, \&
  {Wilson-Hodge}}]{2010ApJ...725..225G}
{Guiriec}, S., {Briggs}, M.~S., {Connaugthon}, V., {et~al.} 2010{\natexlab{a}},
  \apj, 725, 225

\bibitem[{{Guiriec} {et~al.}(2010{\natexlab{b}}){Guiriec}, {Briggs},
  {Connaugthon}, {Kara}, {Daigne}, {Kouveliotou}, {van der Horst}, {Paciesas},
  {Meegan}, {Bhat}, {Foley}, {Bissaldi}, {Burgess}, {Chaplin}, {Diehl},
  {Fishman}, {Gibby}, {Giles}, {Goldstein}, {Greiner}, {Gruber}, {von Kienlin},
  {Kippen}, {McBreen}, {Preece}, {Rau}, {Tierney}, \&
  {Wilson-Hodge}}]{guiriec:2010}
---. 2010{\natexlab{b}}, \apj, 725, 225

\bibitem[{{Guiriec} {et~al.}(2011{\natexlab{a}}){Guiriec}, {Connaughton},
  {Briggs}, {Burgess}, {Ryde}, {Daigne}, {M{\'e}sz{\'a}ros}, {Goldstein},
  {McEnery}, {Omodei}, {Bhat}, {Bissaldi}, {Camero-Arranz}, {Chaplin}, {Diehl},
  {Fishman}, {Foley}, {Gibby}, {Giles}, {Greiner}, {Gruber}, {von Kienlin},
  {Kippen}, {Kouveliotou}, {McBreen}, {Meegan}, {Paciesas}, {Preece}, {Rau},
  {Tierney}, {van der Horst}, \& {Wilson-Hodge}}]{2011ApJ...727L..33G}
{Guiriec}, S., {Connaughton}, V., {Briggs}, M.~S., {et~al.} 2011{\natexlab{a}},
  \apjl, 727, L33

\bibitem[{{Guiriec} {et~al.}(2011{\natexlab{b}}){Guiriec}, {Connaughton},
  {Briggs}, {Burgess}, {Ryde}, {Daigne}, {M{\'e}sz{\'a}ros}, {Goldstein},
  {McEnery}, {Omodei}, {Bhat}, {Bissaldi}, {Camero-Arranz}, {Chaplin}, {Diehl},
  {Fishman}, {Foley}, {Gibby}, {Giles}, {Greiner}, {Gruber}, {von Kienlin},
  {Kippen}, {Kouveliotou}, {McBreen}, {Meegan}, {Paciesas}, {Preece}, {Rau},
  {Tierney}, {van der Horst}, \& {Wilson-Hodge}}]{guiriec:2011}
---. 2011{\natexlab{b}}, \apjl, 727, L33

\bibitem[{{Guiriec} {et~al.}(2013){Guiriec}, {Daigne}, {Hasco{\"e}t},
  {Vianello}, {Ryde}, {Mochkovitch}, {Kouveliotou}, {Xiong}, {Bhat}, {Foley},
  {Gruber}, {Burgess}, {McGlynn}, {McEnery}, \&
  {Gehrels}}]{2013ApJ...770...32G}
{Guiriec}, S., {Daigne}, F., {Hasco{\"e}t}, R., {et~al.} 2013, \apj, 770, 32

\bibitem[{{Guo} \& {Wu}(2010)}]{china:2010}
{Guo}, H., \& {Wu}, J. 2010, Springer-Verlag

\bibitem[{{Gupta} \& {Zhang}(2007)}]{Gupta2007}
{Gupta}, N., \& {Zhang}, B. 2007, Astroparticle Physics, 27, 386

\bibitem[{{Hartoog} {et~al.}(2015){Hartoog}, {Malesani}, {Fynbo}, {Goto},
  {Kr{\"u}hler}, {Vreeswijk}, {De Cia}, {Xu}, {M{\o}ller}, {Covino}, {D'Elia},
  {Flores}, {Goldoni}, {Hjorth}, {Jakobsson}, {Krogager}, {Kaper}, {Ledoux},
  {Levan}, {Milvang-Jensen}, {Sollerman}, {Sparre}, {Tagliaferri}, {Tanvir},
  {de Ugarte Postigo}, {Vergani}, {Wiersema}, {Datson}, {Salinas}, {Mikkelsen},
  \& {Aghanim}}]{2015A&A...580A.139H}
{Hartoog}, O.~E., {Malesani}, D., {Fynbo}, J.~P.~U., {et~al.} 2015, \aap, 580,
  A139

\bibitem[{{Hasco{\"e}t} {et~al.}(2012){Hasco{\"e}t}, {Daigne}, \&
  {Mochkovitch}}]{hascoet:12}
{Hasco{\"e}t}, R., {Daigne}, F., \& {Mochkovitch}, R. 2012, \aap, 542, L29

\bibitem[{{Hasco{\"e}t} {et~al.}(2013){Hasco{\"e}t}, {Daigne}, \&
  {Mochkovitch}}]{hascoet:13}
---. 2013, \aap, 551, A124

\bibitem[{{Hatsukade} {et~al.}(2014){Hatsukade}, {Ohta}, {Endo}, {Nakanishi},
  {Tamura}, {Hashimoto}, \& {Kohno}}]{Hatsukade14}
{Hatsukade}, B., {Ohta}, K., {Endo}, A., {et~al.} 2014, \nat, 510, 247

\bibitem[{{Heger} {et~al.}(2003){Heger}, {Fryer}, {Woosley}, {Langer}, \&
  {Hartmann}}]{2003ApJ...591..288H}
{Heger}, A., {Fryer}, C.~L., {Woosley}, S.~E., {Langer}, N., \& {Hartmann},
  D.~H. 2003, \apj, 591, 288

\bibitem[{{Hern{\'a}ndez-Garc{\'{\i}}a}
  {et~al.}(2015){Hern{\'a}ndez-Garc{\'{\i}}a}, {Masegosa},
  {Gonz{\'a}lez-Mart{\'{\i}}n}, \& {M{\'a}rquez}}]{Hernandez2015}
{Hern{\'a}ndez-Garc{\'{\i}}a}, L., {Masegosa}, J.,
  {Gonz{\'a}lez-Mart{\'{\i}}n}, O., \& {M{\'a}rquez}, I. 2015, \aap, 579, A90

\bibitem[{{Heussaff} {et~al.}(2013){Heussaff}, {Atteia}, \&
  {Zolnierowski}}]{heussaff:2013}
{Heussaff}, V., {Atteia}, J.-L., \& {Zolnierowski}, Y. 2013, \aap, 557, A100

\bibitem[{{Hjorth} \& {Bloom}(2011)}]{Hjorth2011}
{Hjorth}, J., \& {Bloom}, J.~S. 2011, Chapter 9 in "Gamma-Ray Bursts", eds. C.
  Kouveliotou, R. A. M. J. Wijers, S. E. Woosley, Cambridge University Press,
  ArXiv:1104.2274, arXiv:1104.2274

\bibitem[{{Hopkins} \& {Beacom}(2006)}]{2006ApJ...651..142H}
{Hopkins}, A.~M., \& {Beacom}, J.~F. 2006, \apj, 651, 142

\bibitem[{{Hu} {et~al.}(2014){Hu}, {Liang}, {Xi}, {Peng}, {Lu}, {L{\"u}}, \&
  {Zhang}}]{hu2014}
{Hu}, Y.-D., {Liang}, E.-W., {Xi}, S.-Q., {et~al.} 2014, \apj, 789, 145

\bibitem[{{H{\"u}mmer} {et~al.}(2010){H{\"u}mmer}, {R{\"u}ger}, {Spanier}, \&
  {Winter}}]{Hummer2010}
{H{\"u}mmer}, S., {R{\"u}ger}, M., {Spanier}, F., \& {Winter}, W. 2010, \apj,
  721, 630

\bibitem[{{Hunt} {et~al.}(2014){Hunt}, {Palazzi}, {Micha{\l}owski}, {Rossi},
  {Savaglio}, {Basa}, {Berta}, {Bianchi}, {Covino}, {D'Elia}, {Ferrero},
  {G{\"o}tz}, {Greiner}, {Klose}, {Le Borgne}, {Le Floc'h}, {Pian},
  {Piranomonte}, {Schady}, \& {Vergani}}]{hunt14}
{Hunt}, L.~K., {Palazzi}, E., {Micha{\l}owski}, M.~J., {et~al.} 2014, \aap,
  565, A112

\bibitem[{{IceCube Collaboration}(2013)}]{IceCube2013}
{IceCube Collaboration}. 2013, Science, 342, 1242856

\bibitem[{{IceCube Collaboration} {et~al.}(2016){IceCube Collaboration},
  {Aartsen}, {Abraham}, {Ackermann}, {Adams}, {Aguilar}, {Ahlers}, {Ahrens},
  {Altmann}, {Anderson}, \& et~al.}]{IceCube2016}
{IceCube Collaboration}, {Aartsen}, M.~G., {Abraham}, K., {et~al.} 2016, ArXiv
  e-prints, arXiv:1601.06484

\bibitem[{{IceCube-Gen2 Collaboration} {et~al.}(2014){IceCube-Gen2
  Collaboration}, {:}, {Aartsen}, {Ackermann}, {Adams}, {Aguilar}, {Ahlers},
  {Ahrens}, {Altmann}, {Anderson}, \& et~al.}]{ICGen22014}
{IceCube-Gen2 Collaboration}, {:}, {Aartsen}, M.~G., {et~al.} 2014, ArXiv
  e-prints, arXiv:1412.5106

\bibitem[{{Inoue} {et~al.}(2013){Inoue}, {Granot}, {O'Brien}, {Asano},
  {Bouvier}, {Carosi}, {Connaughton}, {Garczarczyk}, {Gilmore}, {Hinton},
  {Inoue}, {Ioka}, {Kakuwa}, {Markoff}, {Murase}, {Osborne}, {Otte},
  {Starling}, {Tajima}, {Teshima}, {Toma}, {Wagner}, {Wijers}, {Williams},
  {Yamamoto}, {Yamazaki}, \& {CTA Consortium}}]{Inoue2013}
{Inoue}, S., {Granot}, J., {O'Brien}, P.~T., {et~al.} 2013, Astroparticle
  Physics, 43, 252

\bibitem[{Inoue {et~al.}(2013)}]{Inoue:2013vy}
Inoue, S., {et~al.} 2013, Astropart. Phys., 43, 252

\bibitem[{{Israel} {et~al.}(2008){Israel}, {Romano}, {Mangano}, {Dall'Osso},
  {Chincarini}, {Stella}, {Campana}, {Belloni}, {Tagliaferri}, {Blustin},
  {Sakamoto}, {Hurley}, {Zane}, {Moretti}, {Palmer}, {Guidorzi}, {Burrows},
  {Gehrels}, \& {Krimm}}]{israel08}
{Israel}, G.~L., {Romano}, P., {Mangano}, V., {et~al.} 2008, \apj, 685, 1114

\bibitem[{{Jakobsson} {et~al.}(2004){Jakobsson}, {Hjorth}, {Fynbo}, {Watson},
  {Pedersen}, {Bj{\"o}rnsson}, \& {Gorosabel}}]{Jakobsson2004}
{Jakobsson}, P., {Hjorth}, J., {Fynbo}, J.~P.~U., {et~al.} 2004, \apjl, 617,
  L21

\bibitem[{{Jin} {et~al.}(2016){Jin}, {Hotokezaka}, {Li}, {Tanaka}, {D'Avanzo},
  {Fan}, {Covino}, {Wei}, \& {Piran}}]{jin:2016}
{Jin}, Z.-P., {Hotokezaka}, K., {Li}, X., {et~al.} 2016, ArXiv e-prints,
  arXiv:1603.07869

\bibitem[{Jonker {et~al.}(2013)}]{Jonker:2013yyp}
Jonker, P., {et~al.} 2013, arXiv:1306.2336

\bibitem[{{Kaneko} {et~al.}(2006{\natexlab{a}}){Kaneko}, {Preece}, {Briggs},
  {Paciesas}, {Meegan}, \& {Band}}]{kaneko:2006}
{Kaneko}, Y., {Preece}, R.~D., {Briggs}, M.~S., {et~al.} 2006{\natexlab{a}},
  \apjs, 166, 298

\bibitem[{{Kaneko} {et~al.}(2006{\natexlab{b}}){Kaneko}, {Preece}, {Briggs},
  {Paciesas}, {Meegan}, \& {Band}}]{2006ApJS..166..298K}
---. 2006{\natexlab{b}}, \apjs, 166, 298

\bibitem[{{Kann} {et~al.}(2011){Kann}, {Klose}, {Zhang}, {Covino}, {Butler},
  {Malesani}, {Nakar}, {Wilson}, {Antonelli}, {Chincarini}, {Cobb}, {D'Avanzo},
  {D'Elia}, {Della Valle}, {Ferrero}, {Fugazza}, {Gorosabel}, {Israel},
  {Mannucci}, {Piranomonte}, {Schulze}, {Stella}, {Tagliaferri}, \&
  {Wiersema}}]{kann:2011}
{Kann}, D.~A., {Klose}, S., {Zhang}, B., {et~al.} 2011, \apj, 734, 96

\bibitem[{{Kawaguchi} {et~al.}(2016){Kawaguchi}, {Kyutoku}, {Shibata}, \&
  {Tanaka}}]{kawaguchi:2016}
{Kawaguchi}, K., {Kyutoku}, K., {Shibata}, M., \& {Tanaka}, M. 2016, ArXiv
  e-prints, arXiv:1601.07711

\bibitem[{{Kelly} {et~al.}(2014){Kelly}, {Filippenko}, {Modjaz}, \&
  {Kocevski}}]{Kelly14}
{Kelly}, P.~L., {Filippenko}, A.~V., {Modjaz}, M., \& {Kocevski}, D. 2014,
  \apj, 789, 23

\bibitem[{{Kisaka} {et~al.}(2016){Kisaka}, {Ioka}, \& {Nakar}}]{kisaka:2016}
{Kisaka}, S., {Ioka}, K., \& {Nakar}, E. 2016, \apj, 818, 104

\bibitem[{{Kistler} {et~al.}(2009){Kistler}, {Y{\"u}ksel}, {Beacom}, {Hopkins},
  \& {Wyithe}}]{kistler09}
{Kistler}, M.~D., {Y{\"u}ksel}, H., {Beacom}, J.~F., {Hopkins}, A.~M., \&
  {Wyithe}, J.~S.~B. 2009, \apjl, 705, L104

\bibitem[{{Kistler} {et~al.}(2008){Kistler}, {Y{\"u}ksel}, {Beacom}, \&
  {Stanek}}]{Kistler2008}
{Kistler}, M.~D., {Y{\"u}ksel}, H., {Beacom}, J.~F., \& {Stanek}, K.~Z. 2008,
  \apjl, 673, L119

\bibitem[{{Klu{\'z}niak} \& {Ruderman}(1998)}]{Klu1998}
{Klu{\'z}niak}, W., \& {Ruderman}, M. 1998, \apjl, 505, L113

\bibitem[{{Kobayashi} {et~al.}(1997){Kobayashi}, {Piran}, \&
  {Sari}}]{kobayashi:97}
{Kobayashi}, S., {Piran}, T., \& {Sari}, R. 1997, \apj, 490, 92

\bibitem[{{Kocevski} \& {Liang}(2006)}]{Kocevski2006}
{Kocevski}, D., \& {Liang}, E. 2006, \apj, 642, 371

\bibitem[{{Kocevski} {et~al.}(2009){Kocevski}, {West}, \&
  {Modjaz}}]{Kocevski2009}
{Kocevski}, D., {West}, A.~A., \& {Modjaz}, M. 2009, \apj, 702, 377

\bibitem[{{Kouveliotou} {et~al.}(1993){Kouveliotou}, {Meegan}, {Fishman},
  {Bhat}, {Briggs}, {Koshut}, {Paciesas}, \& {Pendleton}}]{Kouve93}
{Kouveliotou}, C., {Meegan}, C.~A., {Fishman}, G.~J., {et~al.} 1993, \apjl,
  413, L101

\bibitem[{{Kowalski} \& {Mohr}(2007)}]{IceCube2007}
{Kowalski}, M., \& {Mohr}, A. 2007, Astroparticle Physics, 27, 533

\bibitem[{{Krivonos} {et~al.}(2007{\natexlab{a}}){Krivonos}, {Revnivtsev},
  {Churazov}, {Sazonov}, {Grebenev}, \& {Sunyaev}}]{2007A&A...463..957K}
{Krivonos}, R., {Revnivtsev}, M., {Churazov}, E., {et~al.} 2007{\natexlab{a}},
  \aap, 463, 957

\bibitem[{{Krivonos} {et~al.}(2007{\natexlab{b}}){Krivonos}, {Revnivtsev},
  {Lutovinov}, {Sazonov}, {Churazov}, \& {Sunyaev}}]{krivonos07}
{Krivonos}, R., {Revnivtsev}, M., {Lutovinov}, A., {et~al.} 2007{\natexlab{b}},
  \aap, 475, 775

\bibitem[{{Kr{\"u}hler} {et~al.}(2015){Kr{\"u}hler}, {Malesani}, {Fynbo},
  {Hartoog}, {Hjorth}, {Jakobsson}, {Perley}, {Rossi}, {Schady}, {Schulze},
  {Tanvir}, {Vergani}, {Wiersema}, {Afonso}, {Bolmer}, {Cano}, {Covino},
  {D'Elia}, {de Ugarte Postigo}, {Filgas}, {Friis}, {Graham}, {Greiner},
  {Goldoni}, {Gomboc}, {Hammer}, {Japelj}, {Kann}, {Kaper}, {Klose}, {Levan},
  {Leloudas}, {Milvang-Jensen}, {Nicuesa Guelbenzu}, {Palazzi}, {Pian},
  {Piranomonte}, {S{\'a}nchez-Ram{\'{\i}}rez}, {Savaglio}, {Selsing},
  {Tagliaferri}, {Vreeswijk}, {Watson}, \& {Xu}}]{kruhler15}
{Kr{\"u}hler}, T., {Malesani}, D., {Fynbo}, J.~P.~U., {et~al.} 2015, \aap, 581,
  A125

\bibitem[{{Krumholz}(2012)}]{Krumholz12}
{Krumholz}, M.~R. 2012, \apj, 759, 9

\bibitem[{{Kumar} \& {Zhang}(2015)}]{kumar:2015}
{Kumar}, P., \& {Zhang}, B. 2015, PhR, 561, 1

\bibitem[{{Lacombe} {et~al.}(2014){Lacombe}, {Pons}, {Amoros}, {Atteia},
  {Barret}, {Billot}, {Bordon}, {Cordier}, {Gevin}, {Godet}, {Gonzalez},
  {Houret}, {Mercier}, {Mandrou}, {Marty}, {Nasser}, {Rambaud}, {Ramon},
  {Rouaix}, \& {Waegebaert}}]{Lacombe:14}
{Lacombe}, K., {Pons}, R., {Amoros}, C., {et~al.} 2014, in Proc. SPIE, Vol.
  9144, Space Telescopes and Instrumentation 2014: Ultraviolet to Gamma Ray,
  914451

\bibitem[{{Lapi} {et~al.}(2008){Lapi}, {Kawakatu}, {Bosnjak}, {Celotti},
  {Bressan}, {Granato}, \& {Danese}}]{lapi08}
{Lapi}, A., {Kawakatu}, N., {Bosnjak}, Z., {et~al.} 2008, \mnras, 386, 608

\bibitem[{{Lasky} {et~al.}(2014){Lasky}, {Haskell}, {Ravi}, {Howell}, \&
  {Coward}}]{lasky:2014}
{Lasky}, P.~D., {Haskell}, B., {Ravi}, V., {Howell}, E.~J., \& {Coward}, D.~M.
  2014, \prd, 89, 047302

\bibitem[{{Le} \& {Dermer}(2007)}]{Le2007}
{Le}, T., \& {Dermer}, C.~D. 2007, \apj, 661, 394

\bibitem[{{Le Provost} {et~al.}(2014){Le Provost}, {Schanne}, {Flouzat},
  {Kestener}, {Chaminade}, {Donati}, {Ch{\^a}teau}, {Daly}, \&
  {Fontignie}}]{LeProvost:14}
{Le Provost}, H., {Schanne}, S., {Flouzat}, C., {et~al.} 2014, ArXiv e-prints,
  arXiv:1412.0481

\bibitem[{{Lebrun} {et~al.}(2003){Lebrun}, {Leray}, {Lavocat}, {Cr{\'e}tolle},
  {Arqu{\`e}s}, {Blondel}, {Bonnin}, {Bou{\`e}re}, {Cara}, {Chaleil}, {Daly},
  {Desages}, {Dzitko}, {Horeau}, {Laurent}, {Limousin}, {Mathy}, {Mauguen},
  {Meignier}, {Molini{\'e}}, {Poindron}, {Rouger}, {Sauvageon}, \&
  {Tourrette}}]{Lebrun:03}
{Lebrun}, F., {Leray}, J.~P., {Lavocat}, P., {et~al.} 2003, \aap, 411, L141

\bibitem[{{Lecavelier des Etangs} {et~al.}(2012){Lecavelier des Etangs},
  {Bourrier}, {Wheatley}, {Dupuy}, {Ehrenreich}, {Vidal-Madjar}, {H{\'e}brard},
  {Ballester}, {D{\'e}sert}, {Ferlet}, \& {Sing}}]{lecavelier12}
{Lecavelier des Etangs}, A., {Bourrier}, V., {Wheatley}, P.~J., {et~al.} 2012,
  \aap, 543, L4

\bibitem[{{Ledoux} {et~al.}(2009){Ledoux}, {Vreeswijk}, {Smette}, {Fox},
  {Petitjean}, {Ellison}, {Fynbo}, \& {Savaglio}}]{Ledoux2009}
{Ledoux}, C., {Vreeswijk}, P.~M., {Smette}, A., {et~al.} 2009, \aap, 506, 661

\bibitem[{{Levan} {et~al.}(2006){Levan}, {Wynn}, {Chapman}, {Davies}, {King},
  {Priddey}, \& {Tanvir}}]{levan:2006}
{Levan}, A.~J., {Wynn}, G.~A., {Chapman}, R., {et~al.} 2006, \mnras, 368, L1

\bibitem[{{Levan} {et~al.}(2011){Levan}, {Tanvir}, {Cenko}, {Perley},
  {Wiersema}, {Bloom}, {Fruchter}, {Postigo}, {O'Brien}, {Butler}, {van der
  Horst}, {Leloudas}, {Morgan}, {Misra}, {Bower}, {Farihi}, {Tunnicliffe},
  {Modjaz}, {Silverman}, {Hjorth}, {Th{\"o}ne}, {Cucchiara}, {Cer{\'o}n},
  {Castro-Tirado}, {Arnold}, {Bremer}, {Brodie}, {Carroll}, {Cooper}, {Curran},
  {Cutri}, {Ehle}, {Forbes}, {Fynbo}, {Gorosabel}, {Graham}, {Hoffman},
  {Guziy}, {Jakobsson}, {Kamble}, {Kerr}, {Kasliwal}, {Kouveliotou},
  {Kocevski}, {Law}, {Nugent}, {Ofek}, {Poznanski}, {Quimby}, {Rol},
  {Romanowsky}, {S{\'a}nchez-Ram{\'{\i}}rez}, {Schulze}, {Singh}, {van
  Spaandonk}, {Starling}, {Strom}, {Tello}, {Vaduvescu}, {Wheatley}, {Wijers},
  {Winters}, \& {Xu}}]{levan:11}
{Levan}, A.~J., {Tanvir}, N.~R., {Cenko}, S.~B., {et~al.} 2011, Science, 333,
  199

\bibitem[{{Levan} {et~al.}(2014{\natexlab{a}}){Levan}, {Tanvir}, {Starling},
  {Wiersema}, {Page}, {Perley}, {Schulze}, {Wynn}, {Chornock}, {Hjorth},
  {Cenko}, {Fruchter}, {O'Brien}, {Brown}, {Tunnicliffe}, {Malesani},
  {Jakobsson}, {Watson}, {Berger}, {Bersier}, {Cobb}, {Covino}, {Cucchiara},
  {de Ugarte Postigo}, {Fox}, {Gal-Yam}, {Goldoni}, {Gorosabel}, {Kaper},
  {Kr{\"u}hler}, {Karjalainen}, {Osborne}, {Pian},
  {S{\'a}nchez-Ram{\'{\i}}rez}, {Schmidt}, {Skillen}, {Tagliaferri},
  {Th{\"o}ne}, {Vaduvescu}, {Wijers}, \& {Zauderer}}]{levan:2014a}
{Levan}, A.~J., {Tanvir}, N.~R., {Starling}, R.~L.~C., {et~al.}
  2014{\natexlab{a}}, \apj, 781, 13

\bibitem[{{Levan} {et~al.}(2014{\natexlab{b}}){Levan}, {Tanvir}, {Fruchter},
  {Hjorth}, {Pian}, {Mazzali}, {Hounsell}, {Perley}, {Cano}, {Graham}, {Cenko},
  {Fynbo}, {Kouveliotou}, {Pe'er}, {Misra}, \& {Wiersema}}]{levan:2014}
{Levan}, A.~J., {Tanvir}, N.~R., {Fruchter}, A.~S., {et~al.}
  2014{\natexlab{b}}, \apj, 792, 115

\bibitem[{{Li}(2008)}]{2008MNRAS.388.1487L}
{Li}, L.-X. 2008, \mnras, 388, 1487

\bibitem[{{Li} \& {Paczy{\'n}ski}(1998)}]{li:1998}
{Li}, L.-X., \& {Paczy{\'n}ski}, B. 1998, \apjl, 507, L59

\bibitem[{{Li} \& {Yu}(2016)}]{li:2016}
{Li}, S.-Z., \& {Yu}, Y.-W. 2016, \apj, 819, 120

\bibitem[{{Li} {et~al.}(2016){Li}, {Hu}, {Fan}, \& {Wei}}]{li16}
{Li}, X., {Hu}, Y.-M., {Fan}, Y.-Z., \& {Wei}, D.-M. 2016, ArXiv e-prints,
  arXiv:1601.00180

\bibitem[{{Li} {et~al.}(2002){Li}, {Dai}, \& {Lu}}]{Li2002}
{Li}, Z., {Dai}, Z.~G., \& {Lu}, T. 2002, \aap, 396, 303

\bibitem[{{Liang} \& {Zhang}(2005)}]{2005ApJ...633..611L}
{Liang}, E., \& {Zhang}, B. 2005, \apj, 633, 611

\bibitem[{{Liang} {et~al.}(2007){Liang}, {Zhang}, {Virgili}, \&
  {Dai}}]{liang:2007}
{Liang}, E., {Zhang}, B., {Virgili}, F., \& {Dai}, Z.~G. 2007, \apj, 662, 1111

\bibitem[{{LIGO Scientific Collaboration} {et~al.}(2015){LIGO Scientific
  Collaboration}, {Aasi}, {Abbott}, {Abbott}, {Abbott}, {Abernathy}, {Ackley},
  {Adams}, {Adams}, {Addesso}, \& et~al.}]{aasi:2015}
{LIGO Scientific Collaboration}, {Aasi}, J., {Abbott}, B.~P., {et~al.} 2015,
  Classical and Quantum Gravity, 32, 074001

\bibitem[{{Liu} \& {Wang}(2013)}]{Liu2013}
{Liu}, R.-Y., \& {Wang}, X.-Y. 2013, \apj, 766, 73

\bibitem[{{Lloyd} {et~al.}(2000){Lloyd}, {Petrosian}, \&
  {Mallozzi}}]{2000ApJ...534..227L}
{Lloyd}, N.~M., {Petrosian}, V., \& {Mallozzi}, R.~S. 2000, \apj, 534, 227

\bibitem[{{Lloyd-Ronning} \& {Ramirez-Ruiz}(2002)}]{2002ApJ...576..101L}
{Lloyd-Ronning}, N.~M., \& {Ramirez-Ruiz}, E. 2002, \apj, 576, 101

\bibitem[{{Loeb} \& {Barkana}(2001)}]{2001ARA&A..39...19L}
{Loeb}, A., \& {Barkana}, R. 2001, \araa, 39, 19

\bibitem[{{Lorimer} {et~al.}(2007){Lorimer}, {Bailes}, {McLaughlin},
  {Narkevic}, \& {Crawford}}]{lorimer2007}
{Lorimer}, D.~R., {Bailes}, M., {McLaughlin}, M.~A., {Narkevic}, D.~J., \&
  {Crawford}, F. 2007, Science, 318, 777

\bibitem[{{LSST Science Collaboration} {et~al.}(2009){LSST Science
  Collaboration}, {Abell}, {Allison}, {Anderson}, {Andrew}, {Angel}, {Armus},
  {Arnett}, {Asztalos}, {Axelrod}, \& et~al.}]{lsst:2009}
{LSST Science Collaboration}, {Abell}, P.~A., {Allison}, J., {et~al.} 2009,
  ArXiv e-prints, arXiv:0912.0201

\bibitem[{{L{\"u}} {et~al.}(2010){L{\"u}}, {Liang}, {Zhang}, \&
  {Zhang}}]{lv:2010}
{L{\"u}}, H.-J., {Liang}, E.-W., {Zhang}, B.-B., \& {Zhang}, B. 2010, \apj,
  725, 1965

\bibitem[{{Lynden-Bell}(1971)}]{Lynden-Bell1971}
{Lynden-Bell}, D. 1971, \mnras, 155, 95

\bibitem[{{MacFadyen} \& {Woosley}(1999)}]{Mac1999}
{MacFadyen}, A.~I., \& {Woosley}, S.~E. 1999, \apj, 524, 262

\bibitem[{{Mallozzi} {et~al.}(1995){Mallozzi}, {Paciesas}, {Pendleton},
  {Briggs}, {Preece}, {Meegan}, \& {Fishman}}]{1995ApJ...454..597M}
{Mallozzi}, R.~S., {Paciesas}, W.~S., {Pendleton}, G.~N., {et~al.} 1995, \apj,
  454, 597

\bibitem[{{Martineau-Huynh} {et~al.}(2016){Martineau-Huynh}, {Kotera},
  {Bustamente}, {Charrier}, {De Jong}, {de Vries}, {Fang}, {Feng}, {Finley},
  {Gou}, {Gu}, {Hanson}, {Hu}, {Murase}, {Niess}, {Oikonomou},
  {Renault-Tinacci}, {Schmid}, {Timmermans}, {Wang}, {Wu}, {Zhang}, \&
  {Zhang}}]{Grand2016}
{Martineau-Huynh}, O., {Kotera}, K., {Bustamente}, M., {et~al.} 2016, in
  European Physical Journal Web of Conferences, Vol. 116, European Physical
  Journal Web of Conferences, 03005

\bibitem[{{Mateos} {et~al.}(2008){Mateos}, {Warwick}, {Carrera}, {Stewart},
  {Ebrero}, {Della Ceca}, {Caccianiga}, {Gilli}, {Page}, {Treister}, {Tedds},
  {Watson}, {Lamer}, {Saxton}, {Brunner}, \& {Page}}]{mateos08}
{Mateos}, S., {Warwick}, R.~S., {Carrera}, F.~J., {et~al.} 2008, \aap, 492, 51

\bibitem[{{Mazets} \& {Golenetskii}(1981)}]{mazets:1981}
{Mazets}, E.~P., \& {Golenetskii}, S.~V. 1981, \apss, 75, 47

\bibitem[{{McGuire} {et~al.}(2015){McGuire}, {Tanvir}, {Levan}, {Trenti},
  {Stanway}, {Shull}, {Wiersema}, {Perley}, {Starling}, {Bremer}, {Stocke},
  {Hjorth}, {Rhoads}, {Levesque}, {Robertson}, {Fynbo}, {Ellis}, {Fruchter}, \&
  {Perna}}]{2015arXiv151207808M}
{McGuire}, J.~T.~W., {Tanvir}, N.~R., {Levan}, A.~J., {et~al.} 2015, ArXiv
  e-prints, arXiv:1512.07808

\bibitem[{{Meidinger} {et~al.}(2006){Meidinger}, {Andritschke}, {H{\"a}lker},
  {Hartmann}, {Herrmann}, {Holl}, {Lutz}, {Kimmel}, {Schaller}, {Schnecke},
  {Schopper}, {Soltau}, \& {Str{\"u}der}}]{meidinger}
{Meidinger}, N., {Andritschke}, R., {H{\"a}lker}, O., {et~al.} 2006, Nuclear
  Instruments and Methods in Physics Research A, 568, 141

\bibitem[{{M{\'e}sz{\'a}ros} {et~al.}(2015){M{\'e}sz{\'a}ros}, {Asano},
  {Murase}, {Fox}, {Gao}, \& {Senno}}]{Meszaros2015}
{M{\'e}sz{\'a}ros}, P., {Asano}, K., {Murase}, K., {et~al.} 2015, ArXiv
  e-prints, arXiv:1506.02707

\bibitem[{{M{\'e}sz{\'a}ros} {et~al.}(2002{\natexlab{a}}){M{\'e}sz{\'a}ros},
  {Ramirez-Ruiz}, {Rees}, \& {Zhang}}]{meszaros:02}
{M{\'e}sz{\'a}ros}, P., {Ramirez-Ruiz}, E., {Rees}, M.~J., \& {Zhang}, B.
  2002{\natexlab{a}}, \apj, 578, 812

\bibitem[{{M{\'e}sz{\'a}ros} {et~al.}(2002{\natexlab{b}}){M{\'e}sz{\'a}ros},
  {Ramirez-Ruiz}, {Rees}, \& {Zhang}}]{2002ApJ...578..812M}
---. 2002{\natexlab{b}}, \apj, 578, 812

\bibitem[{{M{\'e}sz{\'a}ros} \& {Rees}(1993)}]{meszaros:93}
{M{\'e}sz{\'a}ros}, P., \& {Rees}, M.~J. 1993, \apjl, 418, L59

\bibitem[{{M{\'e}sz{\'a}ros} \& {Waxman}(2001)}]{Meszaros2001}
{M{\'e}sz{\'a}ros}, P., \& {Waxman}, E. 2001, Physical Review Letters, 87,
  171102

\bibitem[{{Metzger} \& {Berger}(2012)}]{metzger:2012}
{Metzger}, B.~D., \& {Berger}, E. 2012, \apj, 746, 48

\bibitem[{{Micha{\l}owski} {et~al.}(2012){Micha{\l}owski}, {Kamble}, {Hjorth},
  {Malesani}, {Reinfrank}, {Bonavera}, {Castro Cer{\'o}n}, {Ibar}, {Dunlop},
  {Fynbo}, {Garrett}, {Jakobsson}, {Kaplan}, {Kr{\"u}hler}, {Levan},
  {Massardi}, {Pal}, {Sollerman}, {Tanvir}, {van der Horst}, {Watson}, \&
  {Wiersema}}]{michalowski12}
{Micha{\l}owski}, M.~J., {Kamble}, A., {Hjorth}, J., {et~al.} 2012, \apj, 755,
  85

\bibitem[{{Micha{\l}owski} {et~al.}(2015){Micha{\l}owski}, {Gentile}, {Hjorth},
  {Krumholz}, {Tanvir}, {Kamphuis}, {Burlon}, {Baes}, {Basa}, {Berta}, {Castro
  Cer{\'o}n}, {Crosby}, {D'Elia}, {Elliott}, {Greiner}, {Hunt}, {Klose},
  {Koprowski}, {Le Floc'h}, {Malesani}, {Murphy}, {Nicuesa Guelbenzu},
  {Palazzi}, {Rasmussen}, {Rossi}, {Savaglio}, {Schady}, {Sollerman}, {de
  Ugarte Postigo}, {Watson}, {van der Werf}, {Vergani}, \&
  {Xu}}]{Michalowski15}
{Micha{\l}owski}, M.~J., {Gentile}, G., {Hjorth}, J., {et~al.} 2015, \aap, 582,
  A78

\bibitem[{{Middleton} {et~al.}(2013){Middleton}, {Miller-Jones}, {Markoff},
  {Fender}, {Henze}, {Hurley-Walker}, {Scaife}, {Roberts}, {Walton},
  {Carpenter}, {Macquart}, {Bower}, {Gurwell}, {Pietsch}, {Haberl}, {Harris},
  {Daniel}, {Miah}, {Done}, {Morgan}, {Dickinson}, {Charles}, {Burwitz}, {Della
  Valle}, {Freyberg}, {Greiner}, {Hernanz}, {Hartmann}, {Hatzidimitriou},
  {Riffeser}, {Sala}, {Seitz}, {Reig}, {Rau}, {Orio}, {Titterington}, \&
  {Grainge}}]{middleton:13}
{Middleton}, M.~J., {Miller-Jones}, J.~C.~A., {Markoff}, S., {et~al.} 2013,
  \nat, 493, 187

\bibitem[{{Morihana} {et~al.}(2013){Morihana}, {Tsujimoto}, {Yoshida}, \&
  {Ebisawa}}]{2013ApJ...766...14M}
{Morihana}, K., {Tsujimoto}, M., {Yoshida}, T., \& {Ebisawa}, K. 2013, \apj,
  766, 14

\bibitem[{{Motch} {et~al.}(2014){Motch}, {Pakull}, {Soria}, {Gris{\'e}}, \&
  {Pietrzy{\'n}ski}}]{motch:14}
{Motch}, C., {Pakull}, M.~W., {Soria}, R., {Gris{\'e}}, F., \&
  {Pietrzy{\'n}ski}, G. 2014, \nat, 514, 198

\bibitem[{{Murase} \& {Ioka}(2013)}]{Murase2013}
{Murase}, K., \& {Ioka}, K. 2013, Physical Review Letters, 111, 121102

\bibitem[{{Murase} {et~al.}(2006){Murase}, {Ioka}, {Nagataki}, \&
  {Nakamura}}]{Murase2006}
{Murase}, K., {Ioka}, K., {Nagataki}, S., \& {Nakamura}, T. 2006, \apjl, 651,
  L5

\bibitem[{{Murase} {et~al.}(2008){Murase}, {Ioka}, {Nagataki}, \&
  {Nakamura}}]{Murase2008}
---. 2008, \prd, 78, 023005

\bibitem[{{Nasser} {et~al.}(2014){Nasser}, {Godet}, {Atteia}, {Amoros},
  {Barret}, {Bordon}, {Cordier}, {Gevin}, {Gonzalez}, {Houret}, {Lacombe},
  {Mandrou}, {Marty}, {Mercier}, {Pons}, {Rambaud}, {Ramon}, {Rouaix}, \&
  {Waegebaert}}]{Nasser:14}
{Nasser}, G., {Godet}, O., {Atteia}, J.-L., {et~al.} 2014, in Proc. SPIE, Vol.
  9144, Space Telescopes and Instrumentation 2014: Ultraviolet to Gamma Ray,
  91443X

\bibitem[{{Nava} {et~al.}(2011){Nava}, {Ghirlanda}, {Ghisellini}, \&
  {Celotti}}]{2011A&A...530A..21N}
{Nava}, L., {Ghirlanda}, G., {Ghisellini}, G., \& {Celotti}, A. 2011, \aap,
  530, A21

\bibitem[{{Nava} {et~al.}(2006){Nava}, {Ghisellini}, {Ghirlanda}, {Tavecchio},
  \& {Firmani}}]{2006A&A...450..471N}
{Nava}, L., {Ghisellini}, G., {Ghirlanda}, G., {Tavecchio}, F., \& {Firmani},
  C. 2006, \aap, 450, 471

\bibitem[{{Nava} {et~al.}(2012){Nava}, {Salvaterra}, {Ghirlanda}, {Ghisellini},
  {Campana}, {Covino}, {Cusumano}, {D'Avanzo}, {D'Elia}, {Fugazza}, {Melandri},
  {Sbarufatti}, {Vergani}, \& {Tagliaferri}}]{2012MNRAS.421.1256N}
{Nava}, L., {Salvaterra}, R., {Ghirlanda}, G., {et~al.} 2012, \mnras, 421, 1256

\bibitem[{{Norris} \& {Bonnell}(2006)}]{norris:2006}
{Norris}, J.~P., \& {Bonnell}, J.~T. 2006, \apj, 643, 266

\bibitem[{{Norris} {et~al.}(2000){Norris}, {Marani}, \&
  {Bonnell}}]{2000ApJ...534..248N}
{Norris}, J.~P., {Marani}, G.~F., \& {Bonnell}, J.~T. 2000, \apj, 534, 248

\bibitem[{{Noterdaeme} {et~al.}(2015){Noterdaeme}, {Srianand}, {Rahmani},
  {Petitjean}, {P{\^a}ris}, {Ledoux}, {Gupta}, \& {L{\'o}pez}}]{Noterdaeme2015}
{Noterdaeme}, P., {Srianand}, R., {Rahmani}, H., {et~al.} 2015, \aap, 577, A24

\bibitem[{{Ofek} {et~al.}(2007){Ofek}, {Cenko}, {Gal-Yam}, {Fox}, {Nakar},
  {Rau}, {Frail}, {Kulkarni}, {Price}, {Schmidt}, {Soderberg}, {Peterson},
  {Berger}, {Sharon}, {Shemmer}, {Penprase}, {Chevalier}, {Brown}, {Burrows},
  {Gehrels}, {Harrison}, {Holland}, {Mangano}, {McCarthy}, {Moon}, {Nousek},
  {Persson}, {Piran}, \& {Sari}}]{ofek:2007}
{Ofek}, E.~O., {Cenko}, S.~B., {Gal-Yam}, A., {et~al.} 2007, \apj, 662, 1129

\bibitem[{{Olive} {et~al.}(2004){Olive}, {Hurley}, {Sakamoto}, {Atteia},
  {Crew}, {Ricker}, {Pizzichini}, {Barraud}, \& {Kawai}}]{olive04}
{Olive}, J.-F., {Hurley}, K., {Sakamoto}, T., {et~al.} 2004, \apj, 616, 1148

\bibitem[{{Osten} {et~al.}(2010){Osten}, {Godet}, {Drake}, {Tueller},
  {Cummings}, {Krimm}, {Pye}, {Pal'shin}, {Golenetskii}, {Reale}, {Oates},
  {Page}, \& {Melandri}}]{osten2010b}
{Osten}, R.~A., {Godet}, O., {Drake}, S., {et~al.} 2010, \apj, 721, 785

\bibitem[{{Patel} {et~al.}(2010){Patel}, {Warren}, {Mortlock}, \&
  {Fynbo}}]{Patel2010}
{Patel}, M., {Warren}, S.~J., {Mortlock}, D.~J., \& {Fynbo}, J.~P.~U. 2010,
  \aap, 512, L3

\bibitem[{{Paul} {et~al.}(2011){Paul}, {Wei}, {Basa}, \&
  {Zhang}}]{2011CRPhy..12..298P}
{Paul}, J., {Wei}, J., {Basa}, S., \& {Zhang}, S.-N. 2011, Comptes Rendus
  Physique, 12, 298

\bibitem[{{Perley} {et~al.}(2013){Perley}, {Levan}, {Tanvir}, {Cenko}, {Bloom},
  {Hjorth}, {Kr{\"u}hler}, {Filippenko}, {Fruchter}, {Fynbo}, {Jakobsson},
  {Kalirai}, {Milvang-Jensen}, {Morgan}, {Prochaska}, \&
  {Silverman}}]{Perley2013}
{Perley}, D.~A., {Levan}, A.~J., {Tanvir}, N.~R., {et~al.} 2013, \apj, 778, 128

\bibitem[{{Perley} {et~al.}(2016){Perley}, {Tanvir}, {Hjorth}, {Laskar},
  {Berger}, {Chary}, {de Ugarte Postigo}, {Fynbo}, {Kr{\"u}hler}, {Levan},
  {Micha{\l}owski}, \& {Schulze}}]{2016ApJ...817....8P}
{Perley}, D.~A., {Tanvir}, N.~R., {Hjorth}, J., {et~al.} 2016, \apj, 817, 8

\bibitem[{{Perna} \& {Belczynski}(2002)}]{perna:2002}
{Perna}, R., \& {Belczynski}, K. 2002, \apj, 570, 252

\bibitem[{{Pescalli} {et~al.}(2015){Pescalli}, {Ghirlanda}, {Salafia},
  {Ghisellini}, {Nappo}, \& {Salvaterra}}]{2015MNRAS.447.1911P}
{Pescalli}, A., {Ghirlanda}, G., {Salafia}, O.~S., {et~al.} 2015, \mnras, 447,
  1911

\bibitem[{{Pescalli} {et~al.}(2016){Pescalli}, {Ghirlanda}, {Salvaterra},
  {Ghisellini}, {Vergani}, {Nappo}, {Salafia}, {Melandri}, {Covino}, \&
  {G{\"o}tz}}]{pescalli16}
{Pescalli}, A., {Ghirlanda}, G., {Salvaterra}, R., {et~al.} 2016, \aap, 587,
  A40

\bibitem[{{Petitjean} {et~al.}(2006){Petitjean}, {Ledoux}, {Noterdaeme}, \&
  {Srianand}}]{Petitjean2006}
{Petitjean}, P., {Ledoux}, C., {Noterdaeme}, P., \& {Srianand}, R. 2006, \aap,
  456, L9

\bibitem[{{Petitjean} {et~al.}(2016){Petitjean}, {Wang}, {Wu}, \&
  {Wei}}]{Petitjean2016}
{Petitjean}, P., {Wang}, F.~Y., {Wu}, X.~F., \& {Wei}, J.~J. 2016, \ssr,
  arXiv:1601.04279

\bibitem[{{Petrosian} {et~al.}(2015){Petrosian}, {Kitanidis}, \&
  {Kocevski}}]{2015ApJ...806...44P}
{Petrosian}, V., {Kitanidis}, E., \& {Kocevski}, D. 2015, \apj, 806, 44

\bibitem[{{Piran}(1999)}]{piran:1999}
{Piran}, T. 1999, \physrep, 314, 575

\bibitem[{{Qin} {et~al.}(2013){Qin}, {Liang}, {Liang}, {Yi}, {Lin}, {Zhang},
  {Zhang}, {L{\"u}}, {Lu}, {L{\"u}}, \& {Zhang}}]{qin:2013}
{Qin}, Y., {Liang}, E.-W., {Liang}, Y.-F., {et~al.} 2013, \apj, 763, 15

\bibitem[{{Racusin} {et~al.}(2008){Racusin}, {Karpov}, {Sokolowski}, {Granot},
  {Wu}, {Pal'Shin}, {Covino}, {van der Horst}, {Oates}, {Schady}, {Smith},
  {Cummings}, {Starling}, {Piotrowski}, {Zhang}, {Evans}, {Holland}, {Malek},
  {Page}, {Vetere}, {Margutti}, {Guidorzi}, {Kamble}, {Curran}, {Beardmore},
  {Kouveliotou}, {Mankiewicz}, {Melandri}, {O'Brien}, {Page}, {Piran},
  {Tanvir}, {Wrochna}, {Aptekar}, {Barthelmy}, {Bartolini}, {Beskin}, {Bondar},
  {Bremer}, {Campana}, {Castro-Tirado}, {Cucchiara}, {Cwiok}, {D'Avanzo},
  {D'Elia}, {Della Valle}, {de Ugarte Postigo}, {Dominik}, {Falcone}, {Fiore},
  {Fox}, {Frederiks}, {Fruchter}, {Fugazza}, {Garrett}, {Gehrels},
  {Golenetskii}, {Gomboc}, {Gorosabel}, {Greco}, {Guarnieri}, {Immler},
  {Jelinek}, {Kasprowicz}, {La Parola}, {Levan}, {Mangano}, {Mazets},
  {Molinari}, {Moretti}, {Nawrocki}, {Oleynik}, {Osborne}, {Pagani}, {Pandey},
  {Paragi}, {Perri}, {Piccioni}, {Ramirez-Ruiz}, {Roming}, {Steele}, {Strom},
  {Testa}, {Tosti}, {Ulanov}, {Wiersema}, {Wijers}, {Winters}, {Zarnecki},
  {Zerbi}, {M{\'e}sz{\'a}ros}, {Chincarini}, \& {Burrows}}]{racusin2008}
{Racusin}, J.~L., {Karpov}, S.~V., {Sokolowski}, M., {et~al.} 2008, Nature,
  455, 183

\bibitem[{{Rafelski} {et~al.}(2012){Rafelski}, {Wolfe}, {Prochaska},
  {Neeleman}, \& {Mendez}}]{Rafelski2012}
{Rafelski}, M., {Wolfe}, A.~M., {Prochaska}, J.~X., {Neeleman}, M., \&
  {Mendez}, A.~J. 2012, \apj, 755, 89

\bibitem[{{Rahmani} {et~al.}(2013){Rahmani}, {Wendt}, {Srianand}, {Noterdaeme},
  {Petitjean}, {Molaro}, {Whitmore}, {Murphy}, {Centurion}, {Fathivavsari},
  {D'Odorico}, {Evans}, {Levshakov}, {Lopez}, {Martins}, {Reimers}, \&
  {Vladilo}}]{Rahmani2013}
{Rahmani}, H., {Wendt}, M., {Srianand}, R., {et~al.} 2013, \mnras, 435, 861

\bibitem[{{Ramirez-Ruiz} {et~al.}(2002){Ramirez-Ruiz}, {Celotti}, \&
  {Rees}}]{Ram2002}
{Ramirez-Ruiz}, E., {Celotti}, A., \& {Rees}, M.~J. 2002, \mnras, 337, 1349

\bibitem[{{Ramirez-Ruiz} \& {Fenimore}(2000)}]{2000ApJ...539..712R}
{Ramirez-Ruiz}, E., \& {Fenimore}, E.~E. 2000, \apj, 539, 712

\bibitem[{{Raskin} {et~al.}(2008){Raskin}, {Scannapieco}, {Rhoads}, \& {Della
  Valle}}]{Raskin08}
{Raskin}, C., {Scannapieco}, E., {Rhoads}, J., \& {Della Valle}, M. 2008, \apj,
  689, 358

\bibitem[{{Rees} \& {M{\'e}sz{\'a}ros}(1994)}]{rees:94}
{Rees}, M.~J., \& {M{\'e}sz{\'a}ros}, P. 1994, \apjl, 430, L93

\bibitem[{{Rees} \& {M{\'e}sz{\'a}ros}(2005)}]{rees:05}
---. 2005, \apj, 628, 847

\bibitem[{{Reichart} {et~al.}(2001){Reichart}, {Lamb}, {Fenimore},
  {Ramirez-Ruiz}, {Cline}, \& {Hurley}}]{2001ApJ...552...57R}
{Reichart}, D.~E., {Lamb}, D.~Q., {Fenimore}, E.~E., {et~al.} 2001, \apj, 552,
  57

\bibitem[{{Revnivtsev} {et~al.}(2008){Revnivtsev}, {Sazonov}, {Krivonos},
  {Ritter}, \& {Sunyaev}}]{revnivtsev08}
{Revnivtsev}, M., {Sazonov}, S., {Krivonos}, R., {Ritter}, H., \& {Sunyaev}, R.
  2008, \aap, 489, 1121

\bibitem[{{Revnivtsev}(2014)}]{2014AstL...40..667R}
{Revnivtsev}, M.~G. 2014, Astronomy Letters, 40, 667

\bibitem[{{Risaliti} {et~al.}(2011){Risaliti}, {Nardini}, {Salvati}, {Elvis},
  {Fabbiano}, {Maiolino}, {Pietrini}, \& {Torricelli-Ciamponi}}]{Risaliti2011}
{Risaliti}, G., {Nardini}, E., {Salvati}, M., {et~al.} 2011, \mnras, 410, 1027

\bibitem[{{Robertson} \& {Ellis}(2012)}]{robertson12}
{Robertson}, B.~E., \& {Ellis}, R.~S. 2012, \apj, 744, 95

\bibitem[{{Robertson} {et~al.}(2015){Robertson}, {Ellis}, {Furlanetto}, \&
  {Dunlop}}]{2015ApJ...802L..19R}
{Robertson}, B.~E., {Ellis}, R.~S., {Furlanetto}, S.~R., \& {Dunlop}, J.~S.
  2015, \apjl, 802, L19

\bibitem[{{Rodriguez} {et~al.}(2008){Rodriguez}, {Hannikainen}, {Shaw},
  {Pooley}, {Corbel}, {Tagger}, {Mirabel}, {Belloni}, {Cabanac}, {Cadolle Bel},
  {Chenevez}, {Kretschmar}, {Lehto}, {Paizis}, {Varni{\`e}re}, \&
  {Vilhu}}]{rodrigue08_1915a}
{Rodriguez}, J., {Hannikainen}, D.~C., {Shaw}, S.~E., {et~al.} 2008, \apj, 675,
  1436

\bibitem[{{Rodriguez} {et~al.}(2015){Rodriguez}, {Cadolle Bel},
  {Alfonso-Garz{\'o}n}, {Siegert}, {Zhang}, {Grinberg}, {Savchenko}, {Tomsick},
  {Chenevez}, {Clavel}, {Corbel}, {Diehl}, {Domingo}, {Gouiff{\`e}s},
  {Greiner}, {Krause}, {Laurent}, {Loh}, {Markoff}, {Mas-Hesse},
  {Miller-Jones}, {Russell}, \& {Wilms}}]{rodrigue15_V404}
{Rodriguez}, J., {Cadolle Bel}, M., {Alfonso-Garz{\'o}n}, J., {et~al.} 2015,
  \aap, 581, L9

\bibitem[{{Rowlinson} {et~al.}(2013){Rowlinson}, {O'Brien}, {Metzger},
  {Tanvir}, \& {Levan}}]{rowlinson:2013}
{Rowlinson}, A., {O'Brien}, P.~T., {Metzger}, B.~D., {Tanvir}, N.~R., \&
  {Levan}, A.~J. 2013, \mnras, 430, 1061

\bibitem[{{Sakamoto} {et~al.}(2005){Sakamoto}, {Lamb}, {Kawai}, {Yoshida},
  {Graziani}, {Fenimore}, {Donaghy}, {Matsuoka}, {Suzuki}, {Ricker}, {Atteia},
  {Shirasaki}, {Tamagawa}, {Torii}, {Galassi}, {Doty}, {Vanderspek}, {Crew},
  {Villasenor}, {Butler}, {Prigozhin}, {Jernigan}, {Barraud}, {Boer},
  {Dezalay}, {Olive}, {Hurley}, {Levine}, {Monnelly}, {Martel}, {Morgan},
  {Woosley}, {Cline}, {Braga}, {Manchanda}, {Pizzichini}, {Takagishi}, \&
  {Yamauchi}}]{sakamoto:2005}
{Sakamoto}, T., {Lamb}, D.~Q., {Kawai}, N., {et~al.} 2005, \apj, 629, 311

\bibitem[{{Salvaterra}(2015)}]{2015JHEAp...7...35S}
{Salvaterra}, R. 2015, Journal of High Energy Astrophysics, 7, 35

\bibitem[{{Salvaterra} \& {Chincarini}(2007)}]{Salvaterra2007}
{Salvaterra}, R., \& {Chincarini}, G. 2007, \apjl, 656, L49

\bibitem[{{Salvaterra} {et~al.}(2012{\natexlab{a}}){Salvaterra}, {Campana},
  {Vergani}, {Covino}, {D'Avanzo}, {Fugazza}, {Ghirlanda}, {Ghisellini},
  {Melandri}, {Nava}, {Sbarufatti}, {Flores}, {Piranomonte}, \&
  {Tagliaferri}}]{2012ApJ...749...68S}
{Salvaterra}, R., {Campana}, S., {Vergani}, S.~D., {et~al.} 2012{\natexlab{a}},
  \apj, 749, 68

\bibitem[{{Salvaterra} {et~al.}(2012{\natexlab{b}}){Salvaterra}, {Campana},
  {Vergani}, {Covino}, {D'Avanzo}, {Fugazza}, {Ghirlanda}, {Ghisellini},
  {Melandri}, {Nava}, {Sbarufatti}, {Flores}, {Piranomonte}, \&
  {Tagliaferri}}]{salvaterra12}
---. 2012{\natexlab{b}}, \apj, 749, 68

\bibitem[{{Schaefer}(2003)}]{2003ApJ...583L..71S}
{Schaefer}, B.~E. 2003, \apjl, 583, L71

\bibitem[{{Schaefer}(2004)}]{2004ApJ...602..306S}
---. 2004, \apj, 602, 306

\bibitem[{{Schaefer}(2007)}]{2007ApJ...660...16S}
---. 2007, \apj, 660, 16

\bibitem[{{Schanne} {et~al.}(2015){Schanne}, {Cordier}, {Atteia}, {Godet},
  {Lachaud}, \& {Mercier}}]{Schanne:15}
{Schanne}, S., {Cordier}, B., {Atteia}, J.-L., {et~al.} 2015, ArXiv e-prints,
  arXiv:1508.05851

\bibitem[{{Schanne} {et~al.}(2014){Schanne}, {Le Provost}, {Kestener}, {Gros},
  {Cortial}, {G{\"o}tz}, {Sizun}, {Ch{\^a}teau}, \& {Cordier}}]{Schanne:14}
{Schanne}, S., {Le Provost}, H., {Kestener}, P., {et~al.} 2014, ArXiv e-prints,
  arXiv:1411.7810

\bibitem[{{Schechter}(1976)}]{1976ApJ...203..297S}
{Schechter}, P. 1976, \apj, 203, 297

\bibitem[{{Schulze} {et~al.}(2015){Schulze}, {Chapman}, {Hjorth}, {Levan},
  {Jakobsson}, {Bj{\"o}rnsson}, {Perley}, {Kr{\"u}hler}, {Gorosabel}, {Tanvir},
  {de Ugarte Postigo}, {Fynbo}, {Milvang-Jensen}, {M{\o}ller}, \&
  {Watson}}]{schulze15}
{Schulze}, S., {Chapman}, R., {Hjorth}, J., {et~al.} 2015, \apj, 808, 73

\bibitem[{{Skrutskie} {et~al.}(2006){Skrutskie}, {Cutri}, {Stiening},
  {Weinberg}, {Schneider}, {Carpenter}, {Beichman}, {Capps}, {Chester},
  {Elias}, {Huchra}, {Liebert}, {Lonsdale}, {Monet}, {Price}, {Seitzer},
  {Jarrett}, {Kirkpatrick}, {Gizis}, {Howard}, {Evans}, {Fowler}, {Fullmer},
  {Hurt}, {Light}, {Kopan}, {Marsh}, {McCallon}, {Tam}, {Van Dyk}, \&
  {Wheelock}}]{Skrutskie2006}
{Skrutskie}, M.~F., {Cutri}, R.~M., {Stiening}, R., {et~al.} 2006, \aj, 131,
  1163

\bibitem[{{Soldi} {et~al.}(2014){Soldi}, {Beckmann}, {Baumgartner}, {Ponti},
  {Shrader}, {Lubi{\'n}ski}, {Krimm}, {Mattana}, \& {Tueller}}]{Soldi2014}
{Soldi}, S., {Beckmann}, V., {Baumgartner}, W.~H., {et~al.} 2014, \aap, 563,
  A57

\bibitem[{{Soltan}(1982)}]{1982MNRAS.200..115S}
{Soltan}, A. 1982, \mnras, 200, 115

\bibitem[{{Sparre} {et~al.}(2014){Sparre}, {Hartoog}, {Kr{\"u}hler}, {Fynbo},
  {Watson}, {Wiersema}, {D'Elia}, {Zafar}, {Afonso}, {Covino}, {de Ugarte
  Postigo}, {Flores}, {Goldoni}, {Greiner}, {Hjorth}, {Jakobsson}, {Kaper},
  {Klose}, {Levan}, {Malesani}, {Milvang-Jensen}, {Nardini}, {Piranomonte},
  {Sollerman}, {S{\'a}nchez-Ram{\'{\i}}rez}, {Schulze}, {Tanvir}, {Vergani}, \&
  {Wijers}}]{Sparre2014}
{Sparre}, M., {Hartoog}, O.~E., {Kr{\"u}hler}, T., {et~al.} 2014, \apj, 785,
  150

\bibitem[{{Spruit} {et~al.}(2001){Spruit}, {Daigne}, \&
  {Drenkhahn}}]{spruit:01}
{Spruit}, H.~C., {Daigne}, F., \& {Drenkhahn}, G. 2001, \aap, 369, 694

\bibitem[{{Stacy} {et~al.}(2011){Stacy}, {Bromm}, \&
  {Loeb}}]{2011MNRAS.413..543S}
{Stacy}, A., {Bromm}, V., \& {Loeb}, A. 2011, \mnras, 413, 543

\bibitem[{{Stanway} {et~al.}(2015){Stanway}, {Levan}, {Tanvir}, {Wiersema}, \&
  {van der Laan}}]{Stanway15}
{Stanway}, E.~R., {Levan}, A.~J., {Tanvir}, N.~R., {Wiersema}, K., \& {van der
  Laan}, T.~P.~R. 2015, \apjl, 798, L7

\bibitem[{{Steinle}(2010)}]{Steinle2010}
{Steinle}, H. 2010, \pasa, 27, 431

\bibitem[{{Sun} {et~al.}(2015){Sun}, {Zhang}, \& {Li}}]{sun:2015}
{Sun}, H., {Zhang}, B., \& {Li}, Z. 2015, \apj, 812, 33

\bibitem[{{Svensson} {et~al.}(2010){Svensson}, {Levan}, {Tanvir}, {Fruchter},
  \& {Strolger}}]{Svensson2010}
{Svensson}, K.~M., {Levan}, A.~J., {Tanvir}, N.~R., {Fruchter}, A.~S., \&
  {Strolger}, L.-G. 2010, \mnras, 405, 57

\bibitem[{Taboada \& Gilmore(2014{\natexlab{a}})}]{Taboada2013}
Taboada, I., \& Gilmore, R.~C. 2014{\natexlab{a}}, Nucl. Instrum. Meth., A742,
  276

\bibitem[{Taboada \& Gilmore(2014{\natexlab{b}})}]{Taboada:2013uza}
---. 2014{\natexlab{b}}, Nucl. Instrum. Meth., A742, 276

\bibitem[{{Tanvir} {et~al.}(2013){Tanvir}, {Levan}, {Fruchter}, {Hjorth},
  {Hounsell}, {Wiersema}, \& {Tunnicliffe}}]{tanvir:2013}
{Tanvir}, N.~R., {Levan}, A.~J., {Fruchter}, A.~S., {et~al.} 2013, \nat, 500,
  547

\bibitem[{{Tanvir} {et~al.}(2012){Tanvir}, {Levan}, {Fruchter}, {Fynbo},
  {Hjorth}, {Wiersema}, {Bremer}, {Rhoads}, {Jakobsson}, {O'Brien}, {Stanway},
  {Bersier}, {Natarajan}, {Greiner}, {Watson}, {Castro-Tirado}, {Wijers},
  {Starling}, {Misra}, {Graham}, \& {Kouveliotou}}]{2012ApJ...754...46T}
---. 2012, \apj, 754, 46

\bibitem[{{Th{\"o}ne} {et~al.}(2013){Th{\"o}ne}, {Fynbo}, {Goldoni}, {de
  Ugarte}, {Campana}, {Vergani}, {Covino}, {Kr{\"u}hler}, {Kaper}, {Tanvir},
  {Zafar}, {D'Elia}, {Gorosabel}, {Greiner}, {Groot}, {Hammer}, {Jakobsson},
  {Klose}, {Levan}, {Milvang-Jensen}, {Nicuesa}, {Palazzi}, {Piranomonte},
  {Tagliaferri}, {Watson}, {Wiersema}, \& {Wijers}}]{2013MNRAS.428.3590T}
{Th{\"o}ne}, C.~C., {Fynbo}, J.~P.~U., {Goldoni}, P., {et~al.} 2013, \mnras,
  428, 3590

\bibitem[{{Tiengo} {et~al.}(2013){Tiengo}, {Esposito}, {Mereghetti}, {Turolla},
  {Nobili}, {Gastaldello}, {G{\"o}tz}, {Israel}, {Rea}, {Stella}, {Zane}, \&
  {Bignami}}]{tiengo13}
{Tiengo}, A., {Esposito}, P., {Mereghetti}, S., {et~al.} 2013, \nat, 500, 312

\bibitem[{{Tierney} {et~al.}(2013){Tierney}, {McBreen}, {Preece},
  {Fitzpatrick}, {Foley}, {Guiriec}, {Bissaldi}, {Briggs}, {Burgess},
  {Connaughton}, {Goldstein}, {Greiner}, {Gruber}, {Kouveliotou}, {McGlynn},
  {Paciesas}, {Pelassa}, \& {von Kienlin}}]{2013A&A...550A.102T}
{Tierney}, D., {McBreen}, S., {Preece}, R.~D., {et~al.} 2013, \aap, 550, A102

\bibitem[{{Totani}(1997)}]{Totani1997}
{Totani}, T. 1997, \apjl, 486, L71

\bibitem[{{Trenti} {et~al.}(2015){Trenti}, {Perna}, \& {Jimenez}}]{Trenti2015}
{Trenti}, M., {Perna}, R., \& {Jimenez}, R. 2015, \apj, 802, 103

\bibitem[{{Trenti} {et~al.}(2012){Trenti}, {Perna}, {Levesque}, {Shull}, \&
  {Stocke}}]{2012ApJ...749L..38T}
{Trenti}, M., {Perna}, R., {Levesque}, E.~M., {Shull}, J.~M., \& {Stocke},
  J.~T. 2012, \apjl, 749, L38

\bibitem[{{Trenti} {et~al.}(2013){Trenti}, {Perna}, \&
  {Tacchella}}]{Trenti2013}
{Trenti}, M., {Perna}, R., \& {Tacchella}, S. 2013, \apjl, 773, L22

\bibitem[{{T{\"u}rler} {et~al.}(2010){T{\"u}rler}, {Chernyakova},
  {Courvoisier}, {Lubi{\'n}ski}, {Neronov}, {Produit}, \&
  {Walter}}]{2010A&A...512A..49T}
{T{\"u}rler}, M., {Chernyakova}, M., {Courvoisier}, T.~J.-L., {et~al.} 2010,
  \aap, 512, A49

\bibitem[{{Ueda} {et~al.}(2014){Ueda}, {Akiyama}, {Hasinger}, {Miyaji}, \&
  {Watson}}]{Ueda2014}
{Ueda}, Y., {Akiyama}, M., {Hasinger}, G., {Miyaji}, T., \& {Watson}, M.~G.
  2014, \apj, 786, 104

\bibitem[{{van der Horst} {et~al.}(2009){van der Horst}, {Kouveliotou},
  {Gehrels}, {Rol}, {Wijers}, {Cannizzo}, {Racusin}, \&
  {Burrows}}]{van-der-Horst2009}
{van der Horst}, A.~J., {Kouveliotou}, C., {Gehrels}, N., {et~al.} 2009, \apj,
  699, 1087

\bibitem[{{van Haarlem} {et~al.}(2013){van Haarlem}, {Wise}, {Gunst}, {Heald},
  {McKean}, {Hessels}, {de Bruyn}, {Nijboer}, {Swinbank}, {Fallows},
  {Brentjens}, {Nelles}, {Beck}, {Falcke}, {Fender}, {H{\"o}randel},
  {Koopmans}, {Mann}, {Miley}, {R{\"o}ttgering}, {Stappers}, {Wijers},
  {Zaroubi}, {van den Akker}, {Alexov}, {Anderson}, {Anderson}, {van Ardenne},
  {Arts}, {Asgekar}, {Avruch}, {Batejat}, {B{\"a}hren}, {Bell}, {Bell}, {van
  Bemmel}, {Bennema}, {Bentum}, {Bernardi}, {Best}, {B{\^i}rzan}, {Bonafede},
  {Boonstra}, {Braun}, {Bregman}, {Breitling}, {van de Brink}, {Broderick},
  {Broekema}, {Brouw}, {Br{\"u}ggen}, {Butcher}, {van Cappellen}, {Ciardi},
  {Coenen}, {Conway}, {Coolen}, {Corstanje}, {Damstra}, {Davies}, {Deller},
  {Dettmar}, {van Diepen}, {Dijkstra}, {Donker}, {Doorduin}, {Dromer}, {Drost},
  {van Duin}, {Eisl{\"o}ffel}, {van Enst}, {Ferrari}, {Frieswijk}, {Gankema},
  {Garrett}, {de Gasperin}, {Gerbers}, {de Geus}, {Grie{\ss}meier}, {Grit},
  {Gruppen}, {Hamaker}, {Hassall}, {Hoeft}, {Holties}, {Horneffer}, {van der
  Horst}, {van Houwelingen}, {Huijgen}, {Iacobelli}, {Intema}, {Jackson},
  {Jelic}, {de Jong}, {Juette}, {Kant}, {Karastergiou}, {Koers}, {Kollen},
  {Kondratiev}, {Kooistra}, {Koopman}, {Koster}, {Kuniyoshi}, {Kramer},
  {Kuper}, {Lambropoulos}, {Law}, {van Leeuwen}, {Lemaitre}, {Loose}, {Maat},
  {Macario}, {Markoff}, {Masters}, {McFadden}, {McKay-Bukowski}, {Meijering},
  {Meulman}, {Mevius}, {Middelberg}, {Millenaar}, {Miller-Jones}, {Mohan},
  {Mol}, {Morawietz}, {Morganti}, {Mulcahy}, {Mulder}, {Munk}, {Nieuwenhuis},
  {van Nieuwpoort}, {Noordam}, {Norden}, {Noutsos}, {Offringa}, {Olofsson},
  {Omar}, {Orr{\'u}}, {Overeem}, {Paas}, {Pandey-Pommier}, {Pandey}, {Pizzo},
  {Polatidis}, {Rafferty}, {Rawlings}, {Reich}, {de Reijer}, {Reitsma},
  {Renting}, {Riemers}, {Rol}, {Romein}, {Roosjen}, {Ruiter}, {Scaife}, {van
  der Schaaf}, {Scheers}, {Schellart}, {Schoenmakers}, {Schoonderbeek},
  {Serylak}, {Shulevski}, {Sluman}, {Smirnov}, {Sobey}, {Spreeuw}, {Steinmetz},
  {Sterks}, {Stiepel}, {Stuurwold}, {Tagger}, {Tang}, {Tasse}, {Thomas},
  {Thoudam}, {Toribio}, {van der Tol}, {Usov}, {van Veelen}, {van der Veen},
  {ter Veen}, {Verbiest}, {Vermeulen}, {Vermaas}, {Vocks}, {Vogt}, {de Vos},
  {van der Wal}, {van Weeren}, {Weggemans}, {Weltevrede}, {White}, {Wijnholds},
  {Wilhelmsson}, {Wucknitz}, {Yatawatta}, {Zarka}, {Zensus}, \& {van
  Zwieten}}]{vanHaarlem:2013}
{van Haarlem}, M.~P., {Wise}, M.~W., {Gunst}, A.~W., {et~al.} 2013, \aap, 556,
  A2

\bibitem[{{Vangioni} {et~al.}(2016){Vangioni}, {Goriely}, {Daigne}, {Fran{\c
  c}ois}, \& {Belczynski}}]{vangioni:2016}
{Vangioni}, E., {Goriely}, S., {Daigne}, F., {Fran{\c c}ois}, P., \&
  {Belczynski}, K. 2016, \mnras, 455, 17

\bibitem[{{Vangioni} {et~al.}(2015){Vangioni}, {Olive}, {Prestegard}, {Silk},
  {Petitjean}, \& {Mandic}}]{vangioni15b}
{Vangioni}, E., {Olive}, K.~A., {Prestegard}, T., {et~al.} 2015, \mnras, 447,
  2575

\bibitem[{{Vergani} {et~al.}(2015){Vergani}, {Salvaterra}, {Japelj}, {Le
  Floc'h}, {D'Avanzo}, {Fernandez-Soto}, {Kr{\"u}hler}, {Melandri}, {Boissier},
  {Covino}, {Puech}, {Greiner}, {Hunt}, {Perley}, {Petitjean}, {Vinci},
  {Hammer}, {Levan}, {Mannucci}, {Campana}, {Flores}, {Gomboc}, \&
  {Tagliaferri}}]{vergani15}
{Vergani}, S.~D., {Salvaterra}, R., {Japelj}, J., {et~al.} 2015, \aap, 581,
  A102

\bibitem[{{Vestrand} {et~al.}(2014){Vestrand}, {Wren}, {Panaitescu}, {Wozniak},
  {Davis}, {Palmer}, {Vianello}, {Omodei}, {Xiong}, {Briggs}, {Elphick},
  {Paciesas}, \& {Rosing}}]{vestrand2014}
{Vestrand}, W.~T., {Wren}, J.~A., {Panaitescu}, A., {et~al.} 2014, Science,
  343, 38

\bibitem[{{Vietri}(1995)}]{Vietri1995}
{Vietri}, M. 1995, \apj, 453, 883

\bibitem[{{Vietri} \& {Stella}(1999)}]{Viet1999}
{Vietri}, M., \& {Stella}, L. 1999, \apjl, 527, L43

\bibitem[{{Virgili} {et~al.}(2011){Virgili}, {Zhang}, {Nagamine}, \&
  {Choi}}]{Virgili2011}
{Virgili}, F.~J., {Zhang}, B., {Nagamine}, K., \& {Choi}, J.-H. 2011, \mnras,
  417, 3025

\bibitem[{{Virgili} {et~al.}(2013){Virgili}, {Mundell}, {Pal'shin}, {Guidorzi},
  {Margutti}, {Melandri}, {Harrison}, {Kobayashi}, {Chornock}, {Henden},
  {Updike}, {Cenko}, {Tanvir}, {Steele}, {Cucchiara}, {Gomboc}, {Levan},
  {Cano}, {Mottram}, {Clay}, {Bersier}, {Kopa{\v c}}, {Japelj}, {Filippenko},
  {Li}, {Svinkin}, {Golenetskii}, {Hartmann}, {Milne}, {Williams}, {O'Brien},
  {Fox}, \& {Berger}}]{virgili:2013}
{Virgili}, F.~J., {Mundell}, C.~G., {Pal'shin}, V., {et~al.} 2013, \apj, 778,
  54

\bibitem[{{Vreeswijk} {et~al.}(2007){Vreeswijk}, {Ledoux}, {Smette}, {Ellison},
  {Jaunsen}, {Andersen}, {Fruchter}, {Fynbo}, {Hjorth}, {Kaufer}, {M{\o}ller},
  {Petitjean}, {Savaglio}, \& {Wijers}}]{Vreeswijk2007}
{Vreeswijk}, P.~M., {Ledoux}, C., {Smette}, A., {et~al.} 2007, \aap, 468, 83

\bibitem[{{Vreeswijk} {et~al.}(2013){Vreeswijk}, {Ledoux}, {Raassen}, {Smette},
  {De Cia}, {Wo{\'z}niak}, {Fox}, {Vestrand}, \& {Jakobsson}}]{Vreeswijk2013}
{Vreeswijk}, P.~M., {Ledoux}, C., {Raassen}, A.~J.~J., {et~al.} 2013, \aap,
  549, A22

\bibitem[{{Wang}(2013)}]{wang2013}
{Wang}, F.~Y. 2013, \aap, 556, A90

\bibitem[{{Wang} \& {Dai}(2009)}]{Wang2009a}
{Wang}, F.~Y., \& {Dai}, Z.~G. 2009, \mnras, 400, L10

\bibitem[{{Wang} \& {Dai}(2011)}]{Wang2011b}
---. 2011, \apjl, 727, L34

\bibitem[{{Wang} {et~al.}(2015){Wang}, {Dai}, \& {Liang}}]{wang15}
{Wang}, F.~Y., {Dai}, Z.~G., \& {Liang}, E.~W. 2015, NewAR, 67, 1

\bibitem[{{Wang} {et~al.}(2007){Wang}, {Razzaque}, {M{\'e}sz{\'a}ros}, \&
  {Dai}}]{Wang2007}
{Wang}, X.-Y., {Razzaque}, S., {M{\'e}sz{\'a}ros}, P., \& {Dai}, Z.-G. 2007,
  \prd, 76, 083009

\bibitem[{{Waxman}(1995)}]{Waxman1995}
{Waxman}, E. 1995, Physical Review Letters, 75, 386

\bibitem[{{Waxman} \& {Bahcall}(1997)}]{Waxman1997}
{Waxman}, E., \& {Bahcall}, J. 1997, Physical Review Letters, 78, 2292

\bibitem[{{Waxman} \& {Bahcall}(2000)}]{Waxman2000}
{Waxman}, E., \& {Bahcall}, J.~N. 2000, \apj, 541, 707

\bibitem[{{Wehrle} {et~al.}(2012){Wehrle}, {Marscher}, {Jorstad}, {Gurwell},
  {Joshi}, {MacDonald}, {Williamson}, {Agudo}, \& {Grupe}}]{Wehrle2012}
{Wehrle}, A.~E., {Marscher}, A.~P., {Jorstad}, S.~G., {et~al.} 2012, \apj, 758,
  72

\bibitem[{{Wei} {et~al.}(2016){Wei}, {Hao}, {Wu}, \& {Yuan}}]{Wei2016}
{Wei}, J.-J., {Hao}, J.-M., {Wu}, X.-F., \& {Yuan}, Y.-F. 2016, Journal of High
  Energy Astrophysics, 9, 1

\bibitem[{{Wheeler} {et~al.}(2000){Wheeler}, {Yi}, {H{\"o}flich}, \&
  {Wang}}]{Whe2000}
{Wheeler}, J.~C., {Yi}, I., {H{\"o}flich}, P., \& {Wang}, L. 2000, \apj, 537,
  810

\bibitem[{{Wijers} {et~al.}(1998){Wijers}, {Bloom}, {Bagla}, \&
  {Natarajan}}]{Wijers1998}
{Wijers}, R.~A.~M.~J., {Bloom}, J.~S., {Bagla}, J.~S., \& {Natarajan}, P. 1998,
  \mnras, 294, L13

\bibitem[{{Wolf} \& {Podsiadlowski}(2007)}]{Wolf2007}
{Wolf}, C., \& {Podsiadlowski}, P. 2007, \mnras, 375, 1049

\bibitem[{{Woosley}(1993)}]{Woo1993}
{Woosley}, S.~E. 1993, \apj, 405, 273

\bibitem[{{Wu} {et~al.}(2012){Wu}, {Xu}, {Zhang}, \& {Wei}}]{Wu2012}
{Wu}, S.-W., {Xu}, D., {Zhang}, F.-W., \& {Wei}, D.-M. 2012, \mnras, 423, 2627

\bibitem[{{Yang} {et~al.}(2015){Yang}, {Jin}, {Li}, {Covino}, {Zheng},
  {Hotokezaka}, {Fan}, {Piran}, \& {Wei}}]{yang:2015}
{Yang}, B., {Jin}, Z.-P., {Li}, X., {et~al.} 2015, Nature Communications, 6,
  7323

\bibitem[{{Yonetoku} {et~al.}(2004{\natexlab{a}}){Yonetoku}, {Murakami},
  {Nakamura}, {Yamazaki}, {Inoue}, \& {Ioka}}]{Yonetoku2004}
{Yonetoku}, D., {Murakami}, T., {Nakamura}, T., {et~al.} 2004{\natexlab{a}},
  \apj, 609, 935

\bibitem[{{Yonetoku} {et~al.}(2004{\natexlab{b}}){Yonetoku}, {Murakami},
  {Nakamura}, {Yamazaki}, {Inoue}, \& {Ioka}}]{2004ApJ...609..935Y}
---. 2004{\natexlab{b}}, \apj, 609, 935

\bibitem[{{Yu} {et~al.}(2015{\natexlab{a}}){Yu}, {Wang}, {Dai}, \&
  {Cheng}}]{Yu2015}
{Yu}, H., {Wang}, F.~Y., {Dai}, Z.~G., \& {Cheng}, K.~S. 2015{\natexlab{a}},
  \apjs, 218, 13

\bibitem[{{Yu} {et~al.}(2015{\natexlab{b}}){Yu}, {Huang}, {Wu}, {Xu}, \&
  {Geng}}]{YuYB15}
{Yu}, Y.~B., {Huang}, Y.~F., {Wu}, X.~F., {Xu}, M., \& {Geng}, J.~J.
  2015{\natexlab{b}}, \apj, 805, 88

\bibitem[{{Y{\"u}ksel} {et~al.}(2008){Y{\"u}ksel}, {Kistler}, {Beacom}, \&
  {Hopkins}}]{Yuksel2008}
{Y{\"u}ksel}, H., {Kistler}, M.~D., {Beacom}, J.~F., \& {Hopkins}, A.~M. 2008,
  \apjl, 683, L5

\bibitem[{{Zhang}(2006)}]{zhang:2006}
{Zhang}, B. 2006, \nat, 444, 1010

\bibitem[{{Zhang} {et~al.}(2006){Zhang}, {Fan}, {Dyks}, {Kobayashi},
  {M{\'e}sz{\'a}ros}, {Burrows}, {Nousek}, \& {Gehrels}}]{ZhangB2006}
{Zhang}, B., {Fan}, Y.~Z., {Dyks}, J., {et~al.} 2006, \apj, 642, 354

\bibitem[{{Zhang} \& {Yan}(2011)}]{zhang:11}
{Zhang}, B., \& {Yan}, H. 2011, \apj, 726, 90

\bibitem[{{Zhang} {et~al.}(2007){Zhang}, {Zhang}, {Liang}, {Gehrels},
  {Burrows}, \& {M{\'e}sz{\'a}ros}}]{zhang:2007}
{Zhang}, B., {Zhang}, B.-B., {Liang}, E.-W., {et~al.} 2007, \apjl, 655, L25

\bibitem[{{Zhang} {et~al.}(2009){Zhang}, {Zhang}, {Virgili}, {Liang}, {Kann},
  {Wu}, {Proga}, {Lv}, {Toma}, {M{\'e}sz{\'a}ros}, {Burrows}, {Roming}, \&
  {Gehrels}}]{zhang:2009}
{Zhang}, B., {Zhang}, B.-B., {Virgili}, F.~J., {et~al.} 2009, \apj, 703, 1696

\bibitem[{{Zhang} {et~al.}(2014){Zhang}, {Zhang}, {Murase}, {Connaughton}, \&
  {Briggs}}]{zhang:2014}
{Zhang}, B.-B., {Zhang}, B., {Murase}, K., {Connaughton}, V., \& {Briggs},
  M.~S. 2014, \apj, 787, 66

\bibitem[{{Zhang} {et~al.}(2003){Zhang}, {Woosley}, \& {MacFadyen}}]{Zhang2003}
{Zhang}, W., {Woosley}, S.~E., \& {MacFadyen}, A.~I. 2003, \apj, 586, 356

\bibitem[{{Zhao} {et~al.}(2012){Zhao}, {Cordier}, {Sizun}, {Wu}, {Dong},
  {Schanne}, {Song}, \& {Liu}}]{Zhao:12}
{Zhao}, D., {Cordier}, B., {Sizun}, P., {et~al.} 2012, Experimental Astronomy,
  34, 705

%\end{thebibliography}

